Neutral Pion Lifetime Measurements and the QCD Chiral Anomaly

A fundamental property of QCD is the presence of the chiral anomaly, which is the primary component of the $\pi^0\rightarrow\gamma\gamma$ decay amplitude. Based on this anomaly and its small ($\simeq$ 4.5%) chiral correction, a firm prediction of the $\pi^0$ lifetime can be used as a test of QCD at confinement scale energies. The interesting experimental and theoretical histories of the $\pi^0$ meson are reviewed, from discovery to the present era. Experimental results are in agreement with the theoretical prediction, within the current ($\simeq$ 3%) experimental error; however, they are not yet sufficiently precise to test the chiral corrected result, which is a firm QCD prediction and is known to $\simeq$ 1% uncertainty. At this level there exist experimental inconsistencies, which require attention. Possible future work to improve the present precision is suggested.

==> Outline.tex <==

\begin{center}
{\bf\large Outline}
\end{center}
\begin{tabbing}
\noindent 1. Introduction                  \hspace{10cm}                            \= 2\\
\noindent 2. Early Experimental History                                             \> 9\\
\noindent 3. $\pi^0\rightarrow\gamma\gamma$ Decay: Theory                           \> 12\\
\indent 3.1 Early Theoretical History                                               \> 12\\
\indent 3.2 The Adler-Bell-Jackiw Anomaly                                           \> 16\\
\indent 3.3 Alternative Approaches: All Roads Lead to Rome                          \> 23\\
\indent 3.4 Real World Corrections                                                  \> 28\\
\indent 3.5 Other Anomalous Processes                                               \> 32\\
\indent 3.6 Radiative Pion Beta Decay                                               \> 35\\
\indent 3.7 Physics of the Anomaly                                                  \> 38\\
\indent 3.8 Theoretical Summary                                                     \> 43\\
\noindent 4. Measurement of the $\pi^0$ Lifetime: the Particle Data Book            \> 43\\
\indent 4.1 Primakoff Effect Measurements                                           \> 44\\
\indent 4.2 Appendix: $\pi^0\rightarrow\gamma\gamma$ Opening Angle Distributions    \> 50\\
\indent 4.3 The Direct Measurement                                                  \> 52\\
\indent 4.4 $e^+e^-$ Colliding Beam Measurements                                    \> 54\\
\noindent 5. PrimEx Experiment                                                      \> 59\\
\noindent 6. Related Measurements                                                   \> 66\\
\noindent 7. Summary and Outlook                                                    \> 69\\
\indent 7.1 Summary: $\pi^0$ Lifetime Experiments                                   \> 69\\
\indent 7.2 Future Outlook                                                          \> 70\\
\noindent References                                                                \> 73\\                                      
\end{tabbing} 

==> bibliography.tex <==
@article{Beringer:2012,
      author         = "Beringer, J. and others",
      title          = "{Review of Particle Physics (RPP)}",
      collaboration  = "Particle Data Group",
      journal        = "Phys.Rev.",
      volume         = "D86",
      pages          = "010001",
      doi            = "10.1103/PhysRevD.86.010001",
      year           = "2012",
      SLACcitation   = "%%CITATION = PHRVA,D86,010001;%%",
}

 @article{Abouzaid:2008,
      author         = "Abouzaid, E. and others",
      title          = "{Determination of the Parity of the Neutral Pion via the
                        Four-Electron Decay}",
      collaboration  = "KTeV Collaboration",
      journal        = "Phys.Rev.Lett.",
      volume         = "100",
      pages          = "182001",
      doi            = "10.1103/PhysRevLett.100.182001",
      year           = "2008",
      eprint         = "0802.2064",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ex",
      reportNumber   = "FERMILAB-PUB-08-032",
      SLACcitation   = "%%CITATION = ARXIV:0802.2064;%%",
}
 
  @article{rjr-1,
      author         = "Treiman, S.B. and Witten, Edward and Jackiw, R. and
                        Zumino, B.",
      title          = "{CURRENT ALGEBRA AND ANOMALIES}",
      year           = "1986",
      SLACcitation   = "%%CITATION = INSPIRE-231761;%%",
}

@BOOK{book-minimal,
   author = "Donald E. Knuth",
   title = "Seminumerical Algorithms",
   publisher = "Addison-Wesley",
   year = "{\noopsort{1973c}}1981",
}

@article{Bjorken:1965zz,
      author         = "Bjorken, James D. and Drell, Sidney D.",
      title          = "{Relativistic quantum fields}",
      year           = "1965",
      reportNumber   = "ISBN-0070054940",
      SLACcitation   = "%%CITATION = ISBN-0070054940 ETC.;%%",
}

@article{dbj-1,
      author         = "Bjorken, James D. and Drell, Sidney D.",
      title          = "{Relativistic quantum fields}",
      year           = "1965",
      note           = "International Series in Pure and Applied Physics.
                        McGraw-Hill Book Company, New York-St.Louis-San
                        Francisco-Toronto-London-Sydney (ISBN-10: 0-07-005494-0)",
      reportNumber   = "ISBN-0070054940",
      SLACcitation   = "%%CITATION = ISBN-0070054940 ETC.;%%",
}
@BOOK{dbj,
      author         = "Bjorken, James D. and Drell, Sidney D.",
      title          = "{Relativistic quantum fields}",
      publisher = "McGraw-Hill Book Company",
      address =" New York",
      year           = "1965",
      %reportNumber   = "ISBN-0070054940",
      %SLACcitation   = "%%CITATION = ISBN-0070054940 ETC.;%%",
}
@BOOK{rjr,
        author         = "Treiman, S.B. and Witten, Edward and Jackiw, R. and
                        Zumino, B.",
      title          = "{Current  Algebra  and Anomalies}",
      publisher = " World Scientific ", 
      address ="Singapore", 
      year           = "1986",
}

@article{gxr,
      author         = "Donoghue, John F. and Holstein, Barry R.",
      title          = "{PION TRANSITIONS AND MODELS OF CHIRAL SYMMETRY}",
      journal        = "Phys.Rev.",
      volume         = "D40",
      pages          = "2378",
      doi            = "10.1103/PhysRevD.40.2378",
      year           = "1989",
      reportNumber   = "UMHEP-325",
      SLACcitation   = "%%CITATION = PHRVA,D40,2378;%%",
}
  
  @article{uch,
      author         = "Urech, Res",
      title          = "{Virtual photons in chiral perturbation theory}",
      journal        = "Nucl.Phys.",
      volume         = "B433",
      pages          = "234-254",
      doi            = "10.1016/0550-3213(95)90707-N",
      year           = "1995",
      eprint         = "hep-ph/9405341",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "BUTP-94-9",
      SLACcitation   = "%%CITATION = HEP-PH/9405341;%%",
}


@article{rhc,
      author         = "Ametller, L. and Knecht, M. and Talavera, P.",
      title          = "{Electromagnetic corrections to gamma pi+- ---&gt; pi0
                        pi+-}",
      journal        = "Phys.Rev.",
      volume         = "D64",
      pages          = "094009",
      doi            = "10.1103/PhysRevD.64.094009",
      year           = "2001",
      eprint         = "hep-ph/0107127",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      SLACcitation   = "%%CITATION = HEP-PH/0107127;%%",
}
  
  
  @article{khb,
     author         = "Holstein, Barry R.",
     title          = "{Chiral anomaly and gamma 3 pi}",
     journal        = "Phys.Rev.",
     volume         = "D53",
     pages          = "4099-4101",
     doi            = "10.1103/PhysRevD.53.4099",
     year           = "1996",
     eprint         = "hep-ph/9512338",
     archivePrefix  = "arXiv",
     primaryClass   = "hep-ph",
     SLACcitation   = "%%CITATION = HEP-PH/9512338;%%",
}
  
  @article{wzx,
      author         = "Wess, J. and Zumino, B.",
      title          = "{Consequences of anomalous Ward identities}",
      journal        = "Phys.Lett.",
      volume         = "B37",
      pages          = "95",
      doi            = "10.1016/0370-2693(71)90582-X",
      year           = "1971",
      SLACcitation   = "%%CITATION = PHLTA,B37,95;%%",
}

@article{unp,
      author         = "Unterdorfer, Rene and Pichl, Hannes",
      title          = "{On the Radiative Pion Decay}",
      journal        = "Eur.Phys.J.",
      volume         = "C55",
      pages          = "273-283",
      doi            = "10.1140/epjc/s10052-008-0584-8",
      year           = "2008",
      eprint         = "0801.2482",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "PSI-PR-07-05",
      SLACcitation   = "%%CITATION = ARXIV:0801.2482;%%",
}


@article{jgm,
      author         = "Gerard, J.M. and Lahna, T.",
      title          = "{The Asymptotic behavior of the pi0 gamma* gamma*
                        vertex}",
      journal        = "Phys.Lett.",
      volume         = "B356",
      pages          = "381-385",
      doi            = "10.1016/0370-2693(95)00811-X",
      year           = "1995",
      eprint         = "hep-ph/9506255",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "UCL-IPT-95-10",
      SLACcitation   = "%%CITATION = HEP-PH/9506255;%%",
}

@article{kfj,
      author         = "Fujikawa, Kazuo",
      title          = "{Comment on Chiral and Conformal Anomalies}",
      journal        = "Phys.Rev.Lett.",
      volume         = "44",
      pages          = "1733",
      doi            = "10.1103/PhysRevLett.44.1733",
      year           = "1980",
      reportNumber   = "ITP-SB-80-12",
      SLACcitation   = "%%CITATION = PRLTA,44,1733;%%",
}
  
  @article{Gross:2005,
  title = {Nobel Lecture: The discovery of asymptotic freedom and the emergence of QCD},
  month = {Sep},
  journal = {Rev. Mod. Phys.},
  doi = {10.1103/RevModPhys.77.837},
  author = {Gross, David J.},
  year = {2005},
  issue = {3},
  url = {http://link.aps.org/doi/10.1103/RevModPhys.77.837},
  publisher = {American Physical Society},
  pages = {837--849},
  volume = {77}
}

@article{Weinberg,
      author         = "Weinberg, Steven",
      title          = "{Phenomenological Lagrangians}",
      journal        = "Physica",
      volume         = "A96",
      pages          = "327",
      year           = "1979",
      note           = "Festschrift honoring Julian Schwinger on his 60th
                        birthday",
      reportNumber   = "HUTP-78-A051A",
      SLACcitation   = "%%CITATION = PHYSA,A96,327;%%",
}

@article{wit,
      author         = "Witten, Edward",
      title          = "{Current Algebra, Baryons, and Quark Confinement}",
      journal        = "Nucl.Phys.",
      volume         = "B223",
      pages          = "433-444",
      doi            = "10.1016/0550-3213(83)90064-0",
      year           = "1983",
}


@article{atv,
      author         = "Antipov, Yu.M. and Batarin, V.A. and Bezzubov, V.A. and
                        Budanov, N.P. and Gorin, Yu.P. and others",
      title          = "{INVESTIGATION OF gamma ---&gt; 3 pi CHIRAL ANOMALY
                        DURING PION PAIR PRODUCTION BY PIONS IN THE NUCLEAR
                        COULOMB FIELD}",
      journal        = "Phys.Rev.",
      volume         = "D36",
      pages          = "21",
      doi            = "10.1103/PhysRevD.36.21",
      year           = "1987",
}

@article{atw,
      author         = "Antipov, Yu.M. and Batarin, V.A. and Bessubov, V.A. and
                        Budanov, N.P. and Gorin, Yu.P. and others",
      title          = "{EXPERIMENTAL MEASUREMENT OF THE GAMMA ---&gt; 3 PI
                        COUPLING CONSTANT}",
      journal        = "Phys.Rev.Lett.",
      volume         = "56",
      pages          = "796-799",
      doi            = "10.1103/PhysRevLett.56.796",
      year           = "1986",
}

@article{vgp,
      author         = "Venugopal, E.P. and Holstein, Barry R.",
      title          = "{Chiral anomaly and eta - eta-prime mixing}",
      journal        = "Phys.Rev.",
      volume         = "D57",
      pages          = "4397-4402",
      doi            = "10.1103/PhysRevD.57.4397",
      year           = "1998",
      eprint         = "hep-ph/9710382",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
}


  @article{Wilczek:2005,
  title = {Nobel Lecture: Asymptotic freedom: From paradox to paradigm},
  month = {Sep},
  journal = {Rev. Mod. Phys.},
  doi = {10.1103/RevModPhys.77.857},
  author = {Wilczek, Frank},
  year = {2005},
  issue = {3},
  url = {http://link.aps.org/doi/10.1103/RevModPhys.77.857},
  publisher = {American Physical Society},
  pages = {857--870},
  volume = {77}
 }
  @article{Yukawa:1935,
      author         = "Yukawa, Hideki",
      title          = "{On the interaction of elementary particles}",
      journal        = "Proc.Phys.Math.Soc.Jap.",
      volume         = "17",
      pages          = "48-57",
      year           = "1935",
}

@article{Nambu:2009,
      author         = "Nambu, Yoichiro",
      title          = "{Nobel Lecture: Spontaneous symmetry breaking in particle
                        physics: A case of cross fertilization}",
      journal        = "Int.J.Mod.Phys.",
      volume         = "A24",
      pages          = "2371-2377",
      doi            = "10.1142/S0217751X0904590X, 10.1103/RevModPhys.81.1015",
      year           = "2009",
}

@article{Leutwyler:2009,
      author         = "Leutwyler, H.",
      title          = "{Light quark masses}",
      journal        = "PoS",
      volume         = "CD09",
      pages          = "005",
      year           = "2009",
      eprint         = "0911.1416",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
}

@article{Leutwyler:1996,
      author         = "Leutwyler, H.",
      title          = "{The Ratios of the light quark masses}",
      journal        = "Phys.Lett.",
      volume         = "B378",
      pages          = "313-318",
      doi            = "10.1016/0370-2693(96)00386-3",
      year           = "1996",
      eprint         = "hep-ph/9602366",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
}

@BOOK{Perkins:1982,
      author         = "Perkins, D.H.",
      title          = "{Introduction to High Energy Physics}",
     publisher        = "Addison-Wesley Publishing Co.",
     address = " Reading, MA",
     year = "1982",
}

@book{dgh,
      author         = "Donoghue, J.F. and Golowich, E. and Holstein, Barry R.",
      title          = "{Dynamics of the Standard Model}",
           publisher = "Cambridge University Press",
       address = " Cambridge",
      year           = "1992",
}

@book{nmc,
      author         = "Burkardt, M. and  Papavassiliou, V. and  
                        Pate, S.  and Goity, J.",
      title          = "The Structure of the eta-prime Meson. Proceedings,
                        International Workshop, Las Cruces, USA, March, 1996",
     publisher = "World Scientific",
     address = " Singapore",
      year           = "1997",
}

@article{Goldstone:1961,
      author         = "Goldstone, J.",
      title          = "{Field Theories with Superconductor Solutions}",
      journal        = "Nuovo Cim.",
      volume         = "19",
      pages          = "154-164",
      doi            = "10.1007/BF02812722",
      year           = "1961",
}

@article{Plano:1959,
      author         = "Plano, R. and Prodell, A. and Samios, N. and Schwartz, M.
                        and Steinberger, J.",
      title          = "{Parity of the Neutral Pion}",
      journal        = "Phys.Rev.Lett.",
      volume         = "3",
      pages          = "525-527",
      doi            = "10.1103/PhysRevLett.3.525",
      year           = "1959",
}

@article{Bernstein:2009,
      author         = "Bernstein, A.M.",
      title          = "{Lifetime measurement of the pi0 meson and the QCD chiral
                        anomaly}",
      journal        = "PoS",
      volume         = "CD09",
      pages          = "035",
      year           = "2009",
}
 @Article{fum,
     author    = "Fukuda, H. and Miuamoto, Y.",
     title     = "{Title}",
     journal   = "Prog. Theo. Phys.",
     volume    = "4",
     year      = "1949",
     pages     = "49-55",
     doi       = "10.1103/ProgTheoPhys.4.49",
}

@Article{pvii,
     author    = "Gupta, S.N.",
     title     = "{Title}",
     journal   = "Proc. Phys. Soc.",
     volume    = "A66",
     year      = "1953",
     pages     = "129-",
     doi       = "10.1103/ProcPhysSoc.A66.129",
}

@Article{jst,
     author    = "Steinberger, J.",
     title     = "{Title}",
     journal   = "Phys. Rev.",
     volume    = "76",
     year      = "1949",
     pages     = "780-",
     doi       = "10.1103/PhysRev.76.780",
}

@Article{vel,
     author    = "Veltman, M.",
     title     = "{Title}",
     journal   = "Proc. Roy. Soc.",
     volume    = "A301",
     year      = "1967",
     pages     = "107-",
     doi       = "10.1103/ProcRoySoc.A301.107",
}

@Article{srw,
     author    = "Widom, A. and Srivastava, Y.",
     title     = "{Title}",
     journal   = "Am. J. Phys.",
     volume    = "56",
     year      = "1988",
     pages     = "824-",
     doi       = "10.1103/AmJPhys.56.824",
}

@Article{rjk,
     author    = "Jackiw, R.",
     title     = "{Title}",
     journal   = "Helv. Phys. Acta",
     volume    = "59",
     year      = "1986",
     pages     = "835-",
     doi       = "10.1103/HelvPhysActa.59.835",
}

@Article{sit,
     author    = "Tomonaga, Sin-Itiro and Oppenheimer, J. R.",
     title     = "{On Infinite Field Reactions in Quantum Field Theory}",
     journal   = "Phys. Rev.",
     volume    = "74",
     year      = "1948",
     pages     = "224-225",
     doi       = "10.1103/PhysRev.74.224",
     SLACcitation  = "%%CITATION = PHRVA,74,224;%%"
}


@article{gtr,
      author         = "Goldberger, M.L. and Treiman, S.B.",
      title          = "{Decay of the pi meson}",
      journal        = "Phys.Rev.",
      volume         = "110",
      pages          = "1178-1184",
      doi            = "10.1103/PhysRev.110.1178",
      year           = "1958",
}

@article{bej,
      author         = "Bell, J.S. and Jackiw, R.",
      title          = "{A PCAC puzzle: pi0 --&gt; gamma gamma in the sigma
                        model}",
      journal        = "Nuovo Cim.",
      volume         = "A60",
      pages          = "47-61",
      doi            = "10.1007/BF02823296",
      year           = "1969",
}

@article{sdl,
      author         = "Adler, Stephen L.",
      title          = "{Axial vector vertex in spinor electrodynamics}",
      journal        = "Phys.Rev.",
      volume         = "177",
      pages          = "2426-2438",
      doi            = "10.1103/PhysRev.177.2426",
      year           = "1969",
}

@article{sut,
      author         = "Sutherland, D.G.",
      title          = "{Current algebra and some nonstrong mesonic decays}",
      journal        = "Nucl.Phys.",
      volume         = "B2",
      pages          = "433-440",
      doi            = "10.1016/0550-3213(67)90180-0",
      year           = "1967",
}

@article{adb,
      author         = "Adler, Stephen L. and Bardeen, William A.",
      title          = "{Absence of higher order corrections in the anomalous
                        axial vector divergence equation}",
      journal        = "Phys.Rev.",
      volume         = "182",
      pages          = "1517-1536",
      doi            = "10.1103/PhysRev.182.1517",
      year           = "1969",
}

@article{wba,
      author         = "Bardeen, William A.",
      title          = "{Anomalous Ward identities in spinor field theories}",
      journal        = "Phys.Rev.",
      volume         = "184",
      pages          = "1848-1857",
      doi            = "10.1103/PhysRev.184.1848",
      year           = "1969",
}

@article{ioo,
      author         = "Ioffe, B.L. and Oganesian, A.G.",
      title          = "{Axial anomaly and the precise value of the pi0 ---&gt; 2
                        gamma decay width}",
      journal        = "Phys.Lett.",
      volume         = "B647",
      pages          = "389-393",
      doi            = "10.1016/j.physletb.2007.02.021",
      year           = "2007",
      eprint         = "hep-ph/0701077",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
}

@article{amu,
      author         = "Mueller, Alfred H.",
      title          = "{LANDAU LEVELS AND THE PARTONIC INTERPRETATION OF THE
                        AXIAL ANOMALY}",
      journal        = "Phys.Lett.",
      volume         = "B234",
      pages          = "517",
      doi            = "10.1016/0370-2693(90)92050-S",
      year           = "1990",
}

@article{bgh,
      author         = "Goity, J.L. and Bernstein, A.M. and Holstein, B.R.",
      title          = "{The Decay pi0 ---&gt; gamma gamma to next to leading
                        order in chiral perturbation theory}",
      journal        = "Phys.Rev.",
      volume         = "D66",
      pages          = "076014",
      doi            = "10.1103/PhysRevD.66.076014",
      year           = "2002",
      eprint         = "hep-ph/0206007",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
}

@article{kam,
      author         = "Kampf, Karol and Moussallam, Bachir",
      title          = "{Chiral expansions of the pi0 lifetime}",
      journal        = "Phys.Rev.",
      volume         = "D79",
      pages          = "076005",
      doi            = "10.1103/PhysRevD.79.076005",
      year           = "2009",
      eprint         = "0901.4688",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
}

@article{anm,
      author         = "Ananthanarayan, B. and Moussallam, B.",
      title          = "{Electromagnetic corrections in the anomaly sector}",
      journal        = "JHEP",
      volume         = "0205",
      pages          = "052",
      year           = "2002",
      eprint         = "hep-ph/0205232",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
}

@article{Donoghue:1985,
      author         = "Donoghue, J.F. and Holstein, Barry R. and Lin, Y.C.R.",
      title          = "{Chiral Loops in pi0, eta0 ---&gt; gamma gamma and eta
                        eta-prime Mixing}",
      journal        = "Phys.Rev.Lett.",
      volume         = "55",
      pages          = "2766-2769",
      doi            = "10.1103/PhysRevLett.55.2766, 10.1103/PhysRevLett.55.2766",
      year           = "1985",
}

@article{bae,
      author         = "Bar, O. and Wiese, U.J.",
      title          = "{Can one see the number of colors?}",
      journal        = "Nucl.Phys.",
      volume         = "B609",
      pages          = "225-246",
      doi            = "10.1016/S0550-3213(01)00288-7",
      year           = "2001",
      eprint         = "hep-ph/0105258",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
}

@article{jsc,
      author         = "Schwinger, Julian S.",
      title          = "{On gauge invariance and vacuum polarization}",
      journal        = "Phys.Rev.",
      volume         = "82",
      pages          = "664-679",
      doi            = "10.1103/PhysRev.82.664",
      year           = "1951",
}

@article{pvi,
      author         = "Pauli, W. and Villars, F.",
      title          = "{On the Invariant regularization in relativistic quantum
                        theory}",
      journal        = "Rev.Mod.Phys.",
      volume         = "21",
      pages          = "434-444",
      doi            = "10.1103/RevModPhys.21.434",
      year           = "1949",
}

@article{chs,
      author         = "Manohar, Aneesh and Georgi, Howard",
      title          = "{Chiral Quarks and the Nonrelativistic Quark Model}",
      journal        = "Nucl.Phys.",
      volume         = "B234",
      pages          = "189",
      doi            = "10.1016/0550-3213(84)90231-1",
      year           = "1984",
}

@article{chsi,
      author         = "Donoghue, John F. and Golowich, Eugene and Holstein,
                        Barry R.",
      title          = "{KAON DECAYS AND A DETERMINATION OF THE SCALE OF CHIRAL
                        SYMMETRY}",
      journal        = "Phys.Rev.",
      volume         = "D30",
      pages          = "587",
      doi            = "10.1103/PhysRevD.30.587",
      year           = "1984",
}

@article{chl,
      author         = "Gasser, J. and Leutwyler, H.",
      title          = "{Chiral Perturbation Theory to One Loop}",
      journal        = "Annals Phys.",
      volume         = "158",
      pages          = "142",
      doi            = "10.1016/0003-4916(84)90242-2",
      year           = "1984",
}

@article{chl1,
      author         = "Gasser, J. and Leutwyler, H.",
      title          = "{Chiral Perturbation Theory: Expansions in the Mass of
                        the Strange Quark}",
      journal        = "Nucl.Phys.",
      volume         = "B250",
      pages          = "465",
      doi            = "10.1016/0550-3213(85)90492-4",
      year           = "1985",
}

 @article{Gasparian:2004,
      author         = "Gasparian, A.",
      title          = "{A high performance hybrid electromagnetic calorimeter at
                        Jefferson Lab}",
      collaboration  = "PrimEx Collaboration",
      pages          = "109-115",
      year           = "2004",
}

 @article{Martel:2008,
      author         = "Martel, P. and Clinton, E. and McWilliams, R. and
                        Lawrence, D. and Miskimen, R. and others",
      title          = "{Nuclear Targets for a Precision Measurement of the
                        Neutral Pion Radiative Width}",
      journal        = "Nucl.Instrum.Meth.",
      volume         = "A612",
      pages          = "46-49",
      doi            = "10.1016/j.nima.2009.09.063",
      year           = "2009",
      eprint         = "0811.2132",
      archivePrefix  = "arXiv",
      primaryClass   = "nucl-ex",
}



 @Article{Lattes:1947,
     author    = "Lattes, C. M. G. and Muirhead, H. and Occhialini, G. P. S.
                  and Powell, C. F.",
     title     = "{PROCESSES INVOLVING CHARGED MESONS}",
     journal   = "Nature",
     volume    = "159",
     year      = "1947",
     pages     = "694-697",
     SLACcitation  = "%%CITATION = NATUA,159,694;%%"
}

 @Article{Bjorklund:1950,
     author    = "Bjorklund, R. and Crandall, W. E. and Moyer, B. J. and
                  York, H. F.",
     title     = "{High Energy Photons from Proton-Nucleon Collisions}",
     journal   = "Phys. Rev.",
     volume    = "77",
     year      = "1950",
     pages     = "213-218",
     doi       = "10.1103/PhysRev.77.213",
     SLACcitation  = "%%CITATION = PHRVA,77,213;%%"
}

@Article{Panofsky:1950,
     author    = "Panofsky, Wolfgang K. H. and Aamodt, R. Lee and Hadley,
                  James",
     title     = "{The Gamma-Ray Spectrum Resulting from Capture of
                  Negative $\pi$-Mesons in Hydrogen and Deuterium}",
     journal   = "Phys. Rev.",
     volume    = "81",
     year      = "1951",
     pages     = "565-574",
     doi       = "10.1103/PhysRev.81.565",
     SLACcitation  = "%%CITATION = PHRVA,81,565;%%"
}

@Article{Panofsky:1950a,
     author    = "Panofsky, Wolfgang K. H. and Aamodt, Lee and Hadley, James
                  and Phillips, Robert",
     title     = "{THE GAMMA-RAY SPECTRUM RESULTING FROM CAPTURE OF NEGATIVE
                  pi MESONS IN HYDROGEN}",
     journal   = "Phys. Rev.",
     volume    = "80",
     year      = "1950",
     pages     = "94",
     doi       = "10.1103/PhysRev.80.94",
     SLACcitation  = "%%CITATION = PHRVA,80,94;%%"
}

@Article{Steinberger:1950,
     author    = "Steinberger, J. and Panofsky, W. K. H. and Steller, J.",
     title     = "{EVIDENCE FOR THE PRODUCTION OF NEUTRAL MESONS BY
                  PHOTONS}",
     journal   = "Phys. Rev.",
     volume    = "78",
     year      = "1950",
     pages     = "802-805",
     doi       = "10.1103/PhysRev.78.802",
     SLACcitation  = "%%CITATION = PHRVA,78,802;%%"
}

@article{PDB,
      author         = "Nakamura, K. and others",
      title          = "{Review of particle physics}",
      collaboration  = "Particle Data Group",
      journal        = "J.Phys.G",
      volume         = "G37",
      pages          = "075021",
      doi            = "10.1088/0954-3899/37/7A/075021",
      year           = "2010",
}

@MISC{PDB-online,
   author = "Particle Data Group online ",
   note="  http://www.pdg.lbl.gov",
}

@article{PDB-2008,
      author         = "Amsler, C. and others",
      title          = "{Review of Particle Physics}",
      collaboration  = "Particle Data Group",
      journal        = "Phys.Lett.",
      volume         = "B667",
      pages          = "1-1340",
      doi            = "10.1016/j.physletb.2008.07.018",
      year           = "2008",
}

@article{Carlson:1950,
      author         = "Carlson, A.G. and Hooper,J.E. and  King,D.T. ",
      journal        = "Phil. Mag.",
      volume         = "41",
      pages          = "701",
           year           = "1950",
   }
 

@article{Bychkov:2009,
      author         = "Bychkov, M. and Pocanic, D. and VanDevender, B.A. and
                        Baranov, V.A. and Bertl, Wilhelm H. and others",
      title          = "{New Precise Measurement of the Pion Weak Form Factors in
                        pi+ ---&gt; e+ nu gamma Decay}",
      journal        = "Phys.Rev.Lett.",
      volume         = "103",
      pages          = "051802",
      doi            = "10.1103/PhysRevLett.103.051802",
      year           = "2009",
      eprint         = "0804.1815",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ex",
}

@article{Mozley:1950,
      author         = "Mozley, R.F.",
      title          = "{Prpduction of $\pi^{+}$ Mesons by X-Rays as a Function of Atomic Number}",
      journal        = "Phys.Rev.",
      volume         = "80",
      pages          = "493",
      doi            = "PhysRev.80.493",
      year           = "1950",
}

@article{Panofsky:1952,
      author         = "Panofsky, W.K.H. and Steinberger, J.N. and Steller, J.",
      title          = "{FURTHER RESULTS ON THE PRODUCTION OF NEUTRAL MESONS BY
                        PHOTONS}",
      journal        = "Phys.Rev.",
      volume         = "86",
      pages          = "180",
      doi            = "10.1103/PhysRev.86.180",
      year           = "1952",
}

@article{Primakoff:1951,
      author         = "Primakoff,H",
      title          = "{Pr0duction of $\pi^{+}$ Mesons by X-Rays as a Function of Atomic Number}",
      journal        = "Phys.Rev.",
      volume         = "81",
      pages          = "899",
      doi            = "PhysRev.81,899",
      year           = "1951",
}

@Article{Lord:1950,
  title = {Evidence for the Multiple Production of Mesons in a Single Nucleon-Nucleon Collision},
  author = {Lord, J. J. and Fainberg, Joseph  and Schein, Marcel },
  journal = {Phys. Rev.},
  volume = {80},
  number = {6},
  pages = {970--973},
  numpages = {3},
  year = {1950},
  month = {Dec},
  doi = {10.1103/PhysRev.80.970},
  publisher = {American Physical Society}
}

@Article{Lord:1952,
  title = {Narrow Angle Pairs of Particles from Nuclear Interactions},
  author = {Lord, J. J. and Fainberg, Joseph  and Haskin, D. M. and Schein, Marcel },
  journal = {Phys. Rev.},
  volume = {87},
  number = {3},
  pages = {538--539},
  numpages = {1},
  year = {1952},
  month = {Aug},
  doi = {10.1103/PhysRev.87.538},
  publisher = {American Physical Society}
}

@Article{Dalitz:1951,
     author    = "Dalitz, R. H.",
     title     = "{On an alternative decay process for the neutral $\pi$-
                  meson, Letters to the Editor}",
     journal   = "Proc. Phys. Soc.",
     volume    = "A64",
     year      = "1951",
     pages     = "667-669",
     SLACcitation  = "%%CITATION = PPSOA,A64,667;%%"
}

@Article{Schein:1953,
  title = {Production of High-Energy Electron Pairs by Negative Pions in Nuclear Collisions},
  author = {Schein, Marcel  and Fainberg, Joseph  and Haskin, D. M. and Glasser, R. G.},
  journal = {Phys. Rev.},
  volume = {91},
  number = {4},
  pages = {973--980},
  numpages = {7},
  year = {1953},
  month = {Aug},
  doi = {10.1103/PhysRev.91.973},
  publisher = {American Physical Society}
}

@Article{Anand:1953,
     author    = "Anand,B.M.",
     title     = "{Observations on the Lifetime of the Neutral $\pi$ Meson}",
     journal   = "Proc.R. Soc.London A",
     volume    = "220",
     year      = "1953",
     pages     = "183-202",
     SLACcitation  = "%%CITATION = PPSOA,A64,667;%%"
}

@Article{Perkins:1955,
     author    = "Perkins,D.H.",
     title     = "{Corrections}",
     journal   = "Phil.Mag.",
     volume    = "46",
     year      = "1955",
     pages     = "1146",
     SLACcitation  = "%%CITATION = PPSOA,A64,667;%%"
}

@Article{Harris:1957,
  title = {Lifetime of the Neutral Pion},
  author = {Harris, G.  and Orear, J.  and Taylor, S. },
  journal = {Phys. Rev.},
  volume = {106},
  number = {2},
  pages = {327--329},
  numpages = {2},
  year = {1957},
  month = {Apr},
  doi = {10.1103/PhysRev.106.327},
  publisher = {American Physical Society}
}

@Article{Blackie:1960,
  title = {Estimate of the Neutral $\pi{}$-Meson Lifetime},
  author = {Blackie, R. F. and Engler, A.  and Mulvey, J. H.},
  journal = {Phys. Rev. Lett.},
  volume = {5},
  number = {8},
  pages = {384--385},
  numpages = {1},
  year = {1960},
  month = {Oct},
  doi = {10.1103/PhysRevLett.5.384},
  publisher = {American Physical Society}
}

@Article{Glasser:1961,
  title = {Mean Lifetime of the Neutral Pion},
  author = {Glasser, R. G. and Seeman, N.  and Stiller, B. },
  journal = {Phys. Rev.},
  volume = {123},
  number = {3},
  pages = {1014--1020},
  numpages = {6},
  year = {1961},
  month = {Aug},
  doi = {10.1103/PhysRev.123.1014},
  publisher = {American Physical Society}
}

@Article{Shwe:1962,
  title = {Decay of Neutral Pions},
  author = {Shwe, Hla  and Smith, Frances M. and Barkas, Walter H.},
  journal = {Phys. Rev.},
  volume = {125},
  number = {3},
  pages = {1024--1027},
  numpages = {3},
  year = {1962},
  month = {Feb},
  doi = {10.1103/PhysRev.125.1024},
  publisher = {American Physical Society}
}

@Article{Tietge:1962,
  title = {Mean Lifetime of the $\pi{}^{0}$ Meson},
  author = {Tietge, J.  and P\"uschel, W. },
  journal = {Phys. Rev.},
  volume = {127},
  number = {4},
  pages = {1324--1327},
  numpages = {3},
  year = {1962},
  month = {Aug},
  doi = {10.1103/PhysRev.127.1324},
  publisher = {American Physical Society}
}

@article{vonDardel:1963,
      author         = "von Dardel, C. and others",
      title          = "{Mean Life of the Neutral Pion}",
      collaboration  = "CERN",
      journal        = "Phys. Lett.",
      volume         = "4",
      pages          = "51",
      doi            = "10.1088/0954-3899/37/7A/075021",
      year           = "1963",
}

%@MISC{vonDardela},
   %author = "We are using the corrected value for $\tau(\pi^{0})$ ",
   %note = "presented in \cite{Atherton:1985}",}

@article{Morpurgo:1964,
      author         = "Morpurgo,G.",
      title          = "{Theory of the Coulomb Photoprocution of $\pi^{0}$ at HIgh Energy and the Determination of the $\pi^{0}$ Lifetime}",
      journal        = "Nuovo Cimento",
      volume         = "31",
      pages          = "37",
      doi            = "10.1088/0954-3899/37/7A/075021",
      year           = "1964",
}

@article{Faldt:1972,
      author         ="Faldt,G.",
      title          = "{Coherent Production in the Nuclear Coulomb Field}",
      journal        = "Nucl. Phys.",
      volume         = "B43",
      pages          = "591",
      doi            = "10.1088/0954-3899/37/7A/075021",
      year           = "1972",
}

@Article{Gourdin:1971,
     author    = "Gourdin, M.",
     title     = "{High energy production of hadrons in the coulomb field of
                  a nucleus}",
     journal   = "Nucl. Phys.",
     volume    = "B32",
     year      = "1971",
     pages     = "415-428",
     doi       = "10.1016/0550-3213(71)90484-6",
     SLACcitation  = "%%CITATION = NUPHA,B32,415;%%"
}

@Article{Gevorkyan:2009,
     author    = "Gevorkyan, S. and Gasparian, A. and Gan, L. and Larin, I.
                  and Khandaker, M.",
     title     = "{Photoproduction of Pseudoscalar Mesons off Nuclei at
                  Forward Angles}",
     journal   = "Phys. Rev.",
     volume    = "C80",
     year      = "2009",
     pages     = "055201",
     eprint    = "0903.4715",
     archivePrefix = "arXiv",
     primaryClass  =  "hep-ph",
     doi       = "10.1103/PhysRevC.80.055201",
     SLACcitation  = "%%CITATION = 0903.4715;%%"
}

@article{Czyz:2012,
      author         = "Czyz, Henryk and Ivashyn, Sergiy",
      title          = "{EKHARA - new gamma gamma generator}",
      year           = "2012",
   journal  = "arXiv",
     volume   = "hep-ph",
     pages    = "1202.1654",
      SLACcitation   = "%%CITATION = ARXIV:1202.1654;%%",
}

@article{Babusci:2011,
      author         = "Babusci, D. and others",
      title          = "{On the possibility to measure the $\pi^0 to \gamma
                        \gamma$ decay width and the $\gamma^* \gamma to \pi^0$ transition form factor with the KLOE-2 experiment}",
      collaboration  = "KLOE-2 Collaboration",
      journal        = "EPJC",
      volume = "72",
      pages     = "1917",
      year           = "2012",
    % doi            = "10.1140/epjc/s10052-012-1917-1",
     % eprint         = "1109.2461",
     % archivePrefix  = "arXiv",
      %primaryClass   = "hep-ph",
      %SLACcitation   = "%%CITATION = ARXIV:1109.2461;%%",
}


@article{Gevorkyan:2009a,
     author    = "Gevorkyan, S. and Gasparian, A. and Gan, L. and Larin, I. and Khandaker, M.",
     title     = "{Incoherent photoproduction of pseudoscalar mesons off nuclei at forward angles}",
       journal  =    "Particles and Nuclei,Letters",  
            volume = "9",  
     year      = "2012",
  pages = "33",
}



@article{Mosel:2011,
      author         = "Kaskulov, Murat M. and Mosel, Ulrich",
      title          = "{Primakoff production of $\pi^0$, $\eta$ and $\eta'$ in  the Coulomb field of a nucleus}",
             journal  =    "arXiv",  
            volume = "hep-ph",  
       year           = "2011",
    pages       = "1103.2097",
}

@article{Laget:2005,
      author         = "Laget, J.M.",
      title          = "{The Primakoff effect on a proton target}",
      journal        = "Phys.Rev.",
      volume         = "C72",
      pages          = "022202",
      doi            = "10.1103/PhysRevC.72.022202",
      year           = "2005",
      eprint         = "hep-ph/0502233",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
}

@article{Sibirtsev:2009,
      author         = "Sibirtsev, A. and Haidenbauer, J. and Krewald, S. and
                        Meissner, U.G. and Thomas, A.W.",
      title          = "{Neutral pion photoproduction at high energies}",
      journal        = "Eur.Phys.J.",
      volume         = "A41",
      pages          = "71-84",
      doi            = "10.1140/epja/i2009-10771-0",
      year           = "2009",
      eprint         = "0902.1819",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
}
@article{Larin:2010,
      author         = "Larin, I. and others",
      title          = "{A New Measurement of the $\pi^0$ Radiative Decay Width}",
      collaboration  = "PrimEx Collaboration",
      journal        = "Phys.Rev.Lett.",
      volume         = "106",
      pages          = "162303",
      doi            = "10.1103/PhysRevLett.106.162303",
      year           = "2011",
      eprint         = "1009.1681",
      archivePrefix  = "arXiv",
      primaryClass   = "nucl-ex",
}

@MISC{McNulty:2011,
   author = " McNulty,D. ",
   note="private communication",
}

@MISC{PDG:private,
   author = " Arguin, J.F. ",
   note="private communication",
}
@MISC{Friedrich:2011,
   author = " Friedrich,J. ",
   note="private communication",
}

@MISC{Denig:2011,
   author = " Denig,A. ",
   note="private communication",
}
@MISC{PrimEx,
   author = " PrimEx collaboration web page: ",
   note="  http://www.jlab.org/primex/",
}

@MISC{Gasparian:2010,
   author = " Gasparian,A. and others",
   note= "{JLab Exp.  E12-10-011.}"
   %;http://www.jlab.org/exp_prog/proposals/10prop.html(2010)",



@Article{Rodrigues:2010,
     author    = "Rodrigues, T. E. and others",
     title     = "{Nuclear incoherent photoproduction of pi0 and eta from 4
                  to 12 GeV}",
     journal   = "Phys. Rev.",
     volume    = "C82",
     year      = "2010",
     pages     = "024608",
     doi       = "10.1103/PhysRevC.82.024608",
     SLACcitation  = "%%CITATION = PHRVA,C82,024608;%%"
}

@Article{Gan:2010yt,
     author    = "Gan, L. and Gasparian, A. and Gevorkyan, S. and Miskimen,
                  R.",
     title     = "{Comments on 'eta -> gamma gamma Decay Width via the
                  Primakoff Cross Section'}",
     year      = "2010",
     eprint    = "1004.0707",
     archivePrefix = "arXiv",
     primaryClass  =  "nucl-ex",
     SLACcitation  = "%%CITATION = 1004.0707;%%"
}

@Article{Atherton:1985,
     author    = "Atherton, H. W. and others",
     title     = "{DIRECT MEASUREMENT OF THE LIFETIME OF THE NEUTRAL PION}",
     journal   = "Phys. Lett.",
     volume    = "B158",
     year      = "1985",
     pages     = "81-84",
     doi       = "10.1016/0370-2693(85)90744-0",
     SLACcitation  = "%%CITATION = PHLTA,B158,81;%%"
}

@PHDTHESIS{Millikan:1985,
   author = "Barrett C. Milliken",
   title = "A Direct  Measurement of the Lifetime of the Neutral Pion",
   school = "University of Chicago",
   type = "{PhD} Dissertation (unpublished)",
   address = "Enrico Fermi Institute",
   year = "1985",
}

@Article{Browman:1974,
     author    = "Browman, A. and others",
     title     = "{The Decay Width of the Neutral pi Meson}",
     journal   = "Phys. Rev. Lett.",
     volume    = "33",
     year      = "1974",
     pages     = "1400",
     doi       = "10.1103/PhysRevLett.33.1400",
     SLACcitation  = "%%CITATION = PRLTA,33,1400;%%"
}

@Article{Browman:1974a,
     author    = "Browman, A. and others",
     title     = "{The Radiative Width of the eta Meson}",
     journal   = "Phys. Rev. Lett.",
     volume    = "32",
     year      = "1974",
     pages     = "1067",
     doi       = "10.1103/PhysRevLett.32.1067",
     SLACcitation  = "%%CITATION = PRLTA,32,1067;%%"
}



@Article{Bellettini:1965,
     author    = "Bellettini,G.. and others",
     title     = "{Primakoff Effect and  $\pi^{0}$ Lifetime}",
     journal   = "Nuovo Cimento",
     volume    = "40A",
     year      = "1965",
     pages     = "1139",
     doi       = "10.1103/PhysRevLett.32.1067",
     SLACcitation  = "%%CITATION = PRLTA,32,1067;%%"
}

@Article{Bellettini:1970,
     author    = "Bellettini, G. and others",
     title     = "{A new measurement of the pi0 lifetime through the
                  primakoff effect in nuclei}",
     journal   = "Nuovo Cim.",
     volume    = "A66",
     year      = "1970",
     pages     = "243-252",
     doi       = "10.1007/BF02819054",
     SLACcitation  = "%%CITATION = NUCIA,A66,243;%%"
}

@Article{Kryshkin:1970,
     author    = "Kryshkin,V.I. and others",
     title     = "{Primakoff Measurement of the $\pi^{0}$ Lifetime}",
     journal   = "Soviet Physics JETP",
     volume    = "30",
     year      = "1970",
     pages     = "1037",
     doi       = "10.1103/PhysRevLett.32.1067",
     SLACcitation  = "%%CITATION = PRLTA,32,1067;%%"
}

@Article{Williams:1988,
     author    = "Williams, D. and others",
 collaboration = "Crystal Ball",
     title     = "{FORMATION OF THE PSEUDOSCALARS pi0, eta AND eta-prime IN
                  THE REACTION gamma gamma $\to$ gamma gamma}",
     journal   = "Phys. Rev.",
     volume    = "D38",
     year      = "1988",
     pages     = "1365",
     doi       = "10.1103/PhysRevD.38.1365",
     SLACcitation  = "%%CITATION = PHRVA,D38,1365;%%"
}






@Article{Behrend:1991,
     author    = "Behrend, H. J. and others",
 collaboration = "CELLO",
     title     = "{A Measurement of the pi0, eta and eta-prime
                  electromagnetic form-factors}",
     journal   = "Z. Phys.",
     volume    = "C49",
     year      = "1991",
     pages     = "401-410",
     doi       = "10.1007/BF01549692",
     SLACcitation  = "%%CITATION = ZEPYA,C49,401;%%"
}


@Article{Steinberger:1949,
  title = {On the Use of Subtraction Fields and the Lifetimes of Some Types of Meson Decay},
  author = {Steinberger, J. },
  journal = {Phys. Rev.},
  volume = {76},
  number = {8},
  pages = {1180--1186},
  numpages = {6},
  year = {1949},
  month = {Oct},
  doi = {10.1103/PhysRev.76.1180},
  publisher = {American Physical Society}
}

@Article{Miskimen:2011,
title ={Neutral Pion Decay},
author={Miskimen, R},
journal={Ann.  Rev. Nucl. Part. Sci.},
volume={61},
pages={1-21},
numpages={21},
year={2011},
doi={10.1146},
publisher={Annual Reviews}
}



@article{Rodrigues:2008,
  title = {$$\eta${}$\rightarrow${}$\gamma${}$\gamma${}$ Decay Width via the Primakoff Cross Section},
  month = {Jul},
  journal = {Phys. Rev. Lett.},
  doi = {10.1103/PhysRevLett.101.012301},
  author = {Rodrigues, T. E. and Arruda-Neto, J. D. T. and Mesa, J. and Garcia, C. and Shtejer, K. and Dale, D. and Nakagawa, I. and Cole, P. L.},
  year = {2008},
  issue = {1},
  url = {http://link.aps.org/doi/10.1103/PhysRevLett.101.012301},
  numpages = {4},
  publisher = {American Physical Society},
  pages = {012301},
  volume = {101},
}

@article{Behrend:1990,
      author         = "Behrend, H.J. and others",
      title          = "{A Measurement of the pi0, eta and eta-prime
                        electromagnetic form-factors}",
      collaboration  = "CELLO Collaboration",
      journal        = "Z.Phys.",
      volume         = "C49",
      pages          = "401-410",
      doi            = "10.1007/BF01549692",
      year           = "1991",
}



@article{Moskal:2011,
      author         = "Moskal, P.",
      title          = "{Studies of the $\eta$ meson with WASA at COSY and KLOE-2
                        at DA$\Phi$NE}",
      year           = "2011",
      note           = "* Temporary entry *",
  journal        = "arXiv, 1102.5548",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ex",
}

@article{Kampf:2006,
      author         = "Kampf, Karol and Knecht, Marc and Novotny, Jiri",
      title          = "{The Dalitz decay pi0 ---&gt; e+ e- gamma revisited}",
      journal        = "Eur.Phys.J.",
      volume         = "C46",
      pages          = "191-217",
      doi            = "10.1140/epjc/s2005-02466-7",
      year           = "2006",
      eprint         = "hep-ph/0510021",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
}

@article{Farzanpay:1992,
      author         = "Farzanpay, F. and Gumplinger, P. and Stetz, A. and
                        Poutissou, J.M. and Blevis, I. and others",
      title          = "{Measurement of the slope of the pi0 electromagnetic
                        form-factor}",
      journal        = "Phys.Lett.",
      volume         = "B278",
      pages          = "413-418",
      doi            = "10.1016/0370-2693(92)90577-Q",
      year           = "1992",
}

@article{Drees:1992,
  title = {Measurement of the ${$\pi${}}^{0}$ electromagnetic transition form factor},
  month = {Mar},
  journal = {Phys. Rev. D},
  doi = {10.1103/PhysRevD.45.1439},
  author = {Drees, Reena Meijer and Waltham, Chris and Bernasconi, Tiziano and Egli, Stephan and Hermes, Erwin and Muheim, Franz and Niebuhr, Carsten and Pruys, Henk and van der Schaaf, Andries and Bertl, Wilhelm and Grossmann-Handschin, Martin and Lordong, Nicolas and Vermeulen, Detlef and Walter, H. Kristian and Eichler, Ralph and Felawka, Larry and Kozlowski, Tadeusz and Playfer, Stephen and Martino, Jacques},
  year = {1992},
  issue = {5},
  url = {http://link.aps.org/doi/10.1103/PhysRevD.45.1439},
  collaboration = {(SINDRUM I Collaboration)},
  publisher = {American Physical Society},
  pages = {1439--1447},
  volume = {45}
}

@article{Hadjimichael:1989,
      author         = "Hadjimichael, E. and Fallieros, S.",
      title          = "{PRODUCTION OF PI0 IN THE COULOMB FIELD OF NUCLEI BY
                        VIRTUAL PHOTONS FROM ELECTRON SCATTERING}",
      journal        = "Phys.Rev.",
      volume         = "C39",
      pages          = "1438-1445",
      doi            = "10.1103/PhysRevC.39.1438",
      year           = "1989",
}

@article{Christ:2010,
      author         = "Christ, N.H. and Dawson, C. and Izubuchi, T. and Jung, C.
                        and Liu, Q. and others",
      title          = "{The $\eta$ and $\eta^\prime$ mesons from Lattice QCD}",
      journal        = "Phys.Rev.Lett.",
      volume         = "105",
      pages          = "241601",
      doi            = "10.1103/PhysRevLett.105.241601",
      year           = "2010",
      eprint         = "1002.2999",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-lat",
}

@article{Ametller:1992,
      author         = "Ametller, L. and Bijnens, J. and Bramon, A. and Cornet,
                        F.",
      title          = "{Transition form-factors in pi0, eta and eta and
                        eta-prime couplings to gamma gamma}",
      journal        = "Phys.Rev.",
      volume         = "D45",
      pages          = "986-989",
      doi            = "10.1103/PhysRevD.45.986",
      year           = "1992",
}


==> section_Barrymod12_copy.tex <==
%\documentclass[12pt]{article}
%\begin{document}

\section {$\pi^0\rightarrow \gamma\gamma$ Decay:  Theory\label{sec:Theory}}

\subsection{Early Theoretical History}
Just as the experimental study of $\pi^0\rightarrow\gamma\gamma$ took place over
many years, the corresponding theoretical understanding of neutral pion decay
evolved over several decades.  The theoretical examination of the decay amplitude for the mode
$\pi^0\rightarrow\gamma\gamma$ began contemporaneous with the work
on renormalization of quantum electrodynamics (QED).  In 1948
Sin-Itiro Tomonaga sent a letter to J. Robert Oppenheimer, who was
then director of the Institute for Advanced Study in Princeton, in
which he described some of the work that he and his group had been
doing in the area of QED.  This work was subsequently published
as a letter in Physical Review\cite{sit}, in which Tomonaga
described his successful work in dealing with divergences involving
the electron mass and charge. However, he was still having
difficulty dealing with the renormalization of the photon propagator,
in that the photon self-energy diagram shown in Fig. \ref{fig:theory1}a was not
only divergent but also violated gauge invariance, leading to a
nonzero value for the photon mass.  In order to study such issues
further, two of his associates----Hiroshi Fukuda and Yoneji
Miyamoto---undertook a calculation of the process $\pi^0\rightarrow
\gamma\gamma$, which involves the pseudoscalar meson-vector current-vector
current (PVV) triangle diagram shown in Fig. \ref{fig:theory1}b\cite{fum}.
They also examined the axial current-vector current-vector current (AVV)
triangle diagram in Fig. \ref{fig:theory1}c, which is a three-point function
connecting the axial vector current to two photons.  Such triangle diagrams are linearly
divergent, and this problem was dealt with by the use of a
Pauli-Villars regulator\cite{pvi},\cite{pvii}. The calculation raised
interesting problems in that the PVV amplitude was found to be gauge
invariant, while the AVV amplitude was not.

A parallel calculation was undertaken by Jack Steinberger at
Princeton (then a theorist), who was aware of the Fukuda-Miyamoto work and, also using
the Pauli-Villars method, obtained similar results\cite{jst}.
Defining
\begin{equation}
{\cal
L}_{\pi\gamma\gamma}=A_{\pi\gamma\gamma}\pi^0F^{\mu\nu}\tilde{F}_{\mu\nu}
\end{equation}
where
$$F_{\mu\nu}=\partial_\mu A_\nu-\partial_\nu A_\mu$$ is the
electromagnetic field tensor and
$$\tilde{F}_{\mu\nu}={1\over 2}\epsilon_{\mu\nu\alpha\beta}F^{\alpha\beta}$$ is the
dual tensor, Steinberger determined, using a proton loop, that
\begin{equation}
A_{\pi\gamma\gamma}={e^2g_{\pi NN}\over 16\pi^2m_N}\label{eq:kh}
\end{equation}
where $g_{\pi NN}$ is the strong pseudoscalar $\pi NN$ coupling
constant.  Using the Goldberger-Treiman relation\cite{gtr}
\begin{equation}
g_{\pi NN}={m_Ng_A\over F_\pi}
\end{equation}
where $g_A\simeq 1.27$ is the neutron axial decay amplitude and
$F_\pi\simeq 92.2$ MeV is the pion decay constant, Eq. \ref{eq:kh}
can be rewritten as
\begin{equation}
A_{\pi \gamma\gamma}={e^2g_A\over 16\pi^2 F_\pi}
\end{equation}
which is remarkably similar to the value
\begin{equation}
A_{\pi \gamma\gamma}^{anom}={e^2\over 16\pi^2F_\pi}
\end{equation}
predicted by the chiral anomaly, as shown below.  The corresponding decay
rate predicted by Steinberger\cite{jst}
\begin{equation}
\Gamma_{\pi\gamma\gamma}={|A_{\pi\gamma\gamma}|^2 m_\pi^3\over 4\pi}=g_A^2\Gamma_{\pi\gamma\gamma}^{anom}
=g_A^2\times 7.76\,\,{\rm eV}
\end{equation}
is about 60\% larger than the later prediction of the chiral anomaly (and the PDG experimental value).

Julian Schwinger also visited these problems in 1951\cite{jsc}. He
showed how to handle the issues with the photon self-energy, and
confirmed that there were difficulties with the triangle diagrams, but
he did not succeed in resolving them.

\begin{figure}
\begin{center}
\includegraphics
*[width=0.50\linewidth,clip=true]{Barry1.pdf}
\end{center}
\caption{Diagrams considered by early workers: a) vacuum polarization;
b) pseudoscalar to $\gamma\gamma$; c) axial current to $\gamma\gamma$.}
\label{fig:theory1}
\end{figure}

\subsection{The Adler-Bell-Jackiw Anomaly}

The resolution of this problem and its connection with symmetry was
not understood until the late 1960's, when at CERN John Bell and
Roman Jackiw examined the problem of $\pi^0$ decay within the
$\sigma$ model, which is known to obey what we now call chiral
symmetry\cite{bej}. At the time, chiral symmetry was manifested
in the validity of PCAC, which asserts that the divergence of the axial current
\begin{equation}
J^a_{5\mu}(x)=\bar{\psi}(x){1\over 2}\tau_a\gamma_\mu\gamma_5\psi(x)
\end{equation}
can be used as an interpolating field for the pion
\begin{equation}
\partial^\mu J_{5\mu}^a(x)=F_\pi m_\pi^2 \phi_\pi^a(x)\label{eq:kn}
\end{equation}
By this logic the divergence of the axial triangle diagram should be
related to the pion decay triangle diagram, but this was clearly not
the case since the PVV amplitude is gauge invariant while its AVV
analog is not. By a careful analysis within the $\sigma$ model, Bell
and Jackiw were able to show that the origin of the problem is the
breaking of chiral symmetry associated with quantizing the theory.  That is, the
chiral symmetry is valid classically but is destroyed via
quantization---a situation which is called anomalous symmetry
breaking or simply the anomaly.  (At the same time as Bell and
Jackiw were resolving the problem, Steve Adler at the Institute for
Advanced Study came to the same conclusion in his study of spinor
field theory\cite{sdl}, and for this reason the phenomenon is often
called the ABJ anomaly.)

The basic reason underlying this behavior is that, because quantum
field theory involves an infinite number of degrees of freedom, the
short distance properties of the theory do not coincide with what is suggested by
naive manipulations.  That one must be very careful in this region is suggested by
the feature that  a spinor field theory obeys the anticommutation relation
\begin{equation}
\{\psi_a(t,\vec{x}),\psi_b^\dagger
(t,\vec{y})\}=\delta^3(\vec{x}-\vec{y})\delta_{ab}.
\end{equation}
Thus one must deal very carefully with a current such as $J^a_{5\mu}(x)$, which
involves both the field and its conjugate defined at the same point and
can be handled in a variety of ways, but in the end all such methods lead to identical results.

Since the result of all techniques is the same, we shall detail here only the most
intuitive of these procedures---perturbation theory---which was the method employed
by the early investigators. Before examining this calculation, however, we review the
simple symmetry aspects that one might expect.  We consider a simple massless spinor
field carrying charge $e$ coupled to the electromagnetic field, for which the Lagrangian
density is
\begin{equation}
{\cal L}=\bar{\psi}(i\not\!{\partial}-e\not\!\!{A})\psi-{1\over
4}F_{\mu\nu}F^{\mu\nu}
\label{eq:mn}
\end{equation}
We note that this Lagrangian is invariant under a global phase
transformation of the spinor field
\begin{equation}
\psi\rightarrow \exp(i\beta)\psi\equiv {\psi_V}'\label{eq:ku}
\end{equation}
which, by Noether's theorem, leads to a conserved polar-vector
current
\begin{equation}
J_\mu=\bar{\psi}\gamma_\mu\psi\quad{\rm with}\quad \partial^\mu J_\mu=0.
\end{equation}
Alternatively, the Lagrangian of Eq. \ref{eq:mn} is also invariant under a global axial
phase transformation
\begin{equation}
\psi\rightarrow\exp(i\zeta\gamma_5)\psi\equiv {\psi_A}'\label{eq:jn}
\end{equation}
which, by Noether's theorem, leads to a conserved axial-vector
current
\begin{equation}
J_{5\mu}=\bar{\psi}\gamma_\mu\gamma_5\psi\quad{\rm with}\quad \partial^\mu J_{5\mu}=0
\end{equation}

Consider now the three point AVV amplitude, which we designate by
\begin{equation}
T_{\mu\nu\gamma}(q_1,q_2)=-ie^2\int d^4x d^4ye^{-iq_1\cdot
x-iq_2\cdot y}<0|T(J_\mu^{em}(x)J_\nu^{em}(y)J_{5\gamma}(0))|0>
\end{equation}
where it is understood that $q_1^2=q_2^2=0$.  Current conservation
for the vector and axial-vector currents  yields the conditions
\begin{equation}
q_1^\mu T_{\mu\nu\gamma}(q_1,q_2)=q_2^\nu
T_{\mu\nu\gamma}(q_1,q_2)=(q_1+q_2)^\gamma
T_{\mu\nu\gamma}(q_1,q_2)=0\label{eq:hf}
\end{equation}
The requirement that all three conditions in Eq. \ref{eq:hf} be
satisfied then leads to the vanishing of the
$\pi^0\rightarrow\gamma\gamma$ decay amplitude, a result which is
called the Sutherland-Veltman theorem\cite{sut},\cite{vel}. This
result can be demonstrated by writing the most general form for
$T_{\mu\nu\gamma}(q_1,q_2)$ which satisfies the strictures of Bose
symmetry, parity conservation, and gauge invariance
\begin{eqnarray}
T_{\mu\nu\gamma}(q_1,q_2)&=&\epsilon_{\lambda\sigma\alpha\beta}\left[
p_\gamma {g^\lambda}_\mu {g^\sigma}_\nu q_1^\alpha q_2^\beta
G_1(p^2)+\left({g^\sigma}_\mu q_{2\nu}-{g^\sigma}_\nu
q_{1\mu}\right)q_1^\alpha q_2^\beta {g^\lambda}_\gamma
G_2(p^2)\right.\nonumber\\
&+&\left.\left(({g^\sigma}_\mu q_{1\nu}-{g^\sigma}_\nu
q_{2\mu})q_1^\alpha q_2^\beta -{1\over 2}p^2{g^\sigma}_\mu
{g^\alpha}_\nu (q_1-q_2)^\beta\right){g^\lambda}_\gamma
G_3(p^2)\right]\nonumber\\
\quad
\end{eqnarray}
where $p=q_1+q_2$ is the momentum carried by the axial current.
Imposing the condition for axial current conservation yields
the constraint
\begin{equation}
0=p^\gamma
T_{\mu\nu\gamma}(q_1,q_2)=\epsilon_{\mu\nu\alpha\beta}q_1^\alpha
q_2^\beta p^2(G_1(p^2)+G_3(p^2))
\end{equation}
Defining the off-shell $\pi^0\rightarrow\gamma\gamma$ amplitude as
\begin{equation}
<\gamma\gamma|\pi^0>=\epsilon_1^{\mu *} \epsilon_2^{\nu *}
A_{\mu\nu}(q_1,q_2)
\end{equation}
where
\begin{equation}
A_{\mu\nu}(q_1,q_2)= A(p^2)\epsilon_{\mu\nu\alpha\beta}q_1^\alpha
q_2^\beta
\end{equation}
we have, using the Lehmann-Symanzik-Zimmermann reduction\cite{dbj} and Eq. \ref{eq:kn},
\begin{equation}
A(p^2)={(m_\pi^2-p^2)\over F_\pi m_\pi^2}p^2(G_1(p^2)+G_3(p^2)).
\end{equation}
Unless  $G_1(p^2)$ and $G_2(p^2)$ develop poles at $p^2=0$, which is excluded on
physical grounds, we conclude that $A(0)=0$, which is the content of the Sutherland-Veltman
theorem, and asserts that in the chiral symmetric limit, where $m_\pi^2=0$,
the $\pi^0\rightarrow\gamma\gamma$ decay amplitude vanishes.  Of course,
in the real world $m_\pi^2\neq 0$ and we must extrapolate from the
chiral limit. However, this scenario would suggest a decay amplitude
of size
\begin{equation}
A(m_\pi^2)\sim {e^2\over 16\pi^2 F_\pi}\times {m_\pi^2\over
\Lambda_\chi^2}\label{eq:bh}
\end{equation}
where $\Lambda_\chi\sim 4\pi F_\pi\sim 1$ GeV is the chiral
scale\cite{chs},\cite{chsi}.  Here the factor $m_\pi^2/\Lambda_\chi^2$ represents the
feature that this amplitude is {\it two} chiral orders higher than the vanishing lowest
order term, the factor $e^2/4\pi$ is needed because we have a two photon amplitude with a loop
diagram, and the "extra" $4\pi F_\pi$ is required for dimensional purposes.  In any case, Eq.
\ref{eq:bh} would lead to a $\pi^0$ lifetime
\begin{equation}
\tau_{\pi^0\rightarrow\gamma\gamma}=1/\Gamma_{\pi^0\rightarrow\gamma\gamma}\sim
10^{-13}\,{\rm s},
\end{equation}
{\it three} orders of magnitude longer than observed.

\begin{figure}
\begin{center}
\includegraphics*[width=0.50\linewidth,clip=true]{Barry2_v3.pdf}
\end{center}
\caption{Perturbation theory diagrams for PVV and AVV processes.  Here the indices
$\mu,\nu$ are Lorentz indices of vector currents while $\gamma$ is the Lorentz index of
the axial-vector current.
\label{fig:theory2}}
\end{figure}

In order to study this phenomenon further we shall examine the
$\pi^0$ decay process in perturbation theory, wherein the
three point function is described by the Feynman diagram in Fig.
\ref{fig:theory2}b
\begin{equation}
T_{\mu\nu\gamma}(q_1,q_2)=U_{\mu\nu\gamma}(q_1,q_2)+U_{\nu\mu\gamma}(q_2,q_1)
\end{equation}
where
\begin{equation}
U_{\mu\nu\gamma}(q_1,q_2)=-i{e^2K_F\over 2}\int{d^4s\over
(2\pi)^4}{\rm Tr}\left({1\over
\not\!{s}+\not\!{q}_1}\gamma_\mu{1\over \not\!{s}}\gamma_\nu{1\over
\not\!{s}-\not\!{q}_2}\gamma_\gamma\gamma_5\right)
\end{equation}
Note that $U_{\mu\nu\gamma}(q_1,q_2)$ arises from
colored quark loops and includes a factor
\begin{equation}
K_F=N_c\sum_{u,d}Q_q^2\tau_{3q}=3\left[({2\over 3})^2-(-{1\over
3})^2\right]=1
\end{equation}
This proportionality of the decay amplitude to $N_c$ has led many
authors to assert that the agreement between experimental and
theoretical values of the $\pi^0\rightarrow\gamma\gamma$ decay rates
offers "proof" that $N_c=3$.  However, Baer and Wiese\cite{bae} and earlier Gerard and
Lahna\cite{jgm} have noted
that anomaly cancelation {\it in a gauge theory} requires, in a two-flavor picture with
$N_c$ colors, that the $u,d$ quark charges must have the values
\begin{equation}
Q_u={1\over 2}[{1\over N_c}+1]\quad{\rm and}\quad Q_d={1\over
2}[{1\over N_c}-1]
\end{equation}
so that the factor $K_F$ has the value
\begin{equation}
K_F={N_c\over 4}[({1\over N_c}+1)^2-({1\over N_c}-1)^2]=1
\end{equation}
in {\it any} consistent theory.  Note that the Steinberger
calculation\cite{jst} is then a special case wherein $N_c=1$ and this feature
is the reason that his calculation agrees with the usual quark model
result.  (Of course, if one also examines other anomalous processes
such as $\eta^0\rightarrow\pi^+\pi^-\gamma$ agreement between
experiment and theory {\it does} require $N_c=3$, and this provides
the real proof.)

We can now check the validity of the various conservation
conditions---Eq. \ref{eq:hf}, the first of which reads
\begin{eqnarray}
q_1^\mu T_{\mu\nu\gamma}(q_1,q_2)&=&-{ie^2\over 2}\int{d^4s\over
(2\pi)^4}{\rm Tr}\left[({1\over \not\!{s}}-{1\over
\not\!{s}+\not\!{q}_1})\gamma_\nu{1\over
\not\!{s}-\not\!{q}_2}\gamma_\gamma\gamma_5\right.\nonumber\\
&+&\left.{1\over \not\!{s}+\not\!{q}_2}\gamma_\nu({1\over
\not\!{s}}-{1\over
\not\!{s}-\not\!{q}_1})\gamma_\gamma\gamma_5\right]
\end{eqnarray}
However, the integrals which involve a {\it single} factor of photon
momentum $q_1$ or $q_2$ vanish, since the epsilon tensor associated
with the trace
$${\rm Tr}\gamma_\mu\gamma_\nu\gamma_\alpha\gamma_\beta\gamma_5=4i\epsilon_{\mu\nu\alpha\beta},$$
requires contraction with {\it two} independent momenta in order
to be nonvanishing.  Thus, defining
\begin{equation}
W_{\nu\gamma}(s)={\rm Tr}\left({1\over \not\!{s}}\gamma_\nu{1\over
\not\!{s}-\not\!{q}_1-\not\!{q}_2}\gamma_\gamma\gamma_5\right)
\end{equation}
we have
\begin{equation}
q_1^\mu T_{\mu\nu\gamma}(q_1,q_2)=-{ie^2\over 2}\int{d^4s\over
(2\pi)^4}[W_{\nu\gamma}(s+q_1)-W_{\nu\gamma}(s+q_2)]\label{eq:dg}
\end{equation}
If the integrals in Eq. \ref{eq:dg} were convergent, or diverged no
worse than logarithmically, then we could shift the integration
variables freely, thereby obtaining zero and verifying gauge invariance.  However,
because there exists a {\it linear} divergence at large $s$ we must be
more careful.  Using Taylor's theorem
\begin{equation}
\int{d^4s\over (2\pi)^4}F(s+a)=\int{d^4s\over
(2\pi)^4}\left[F(s)+a^\alpha\partial_\alpha F(s)+\ldots\right]
\end{equation}
we can write
\begin{equation}
q_1^\mu T_{\mu\nu\gamma}(q_1,q_2)=-{ie^2\over
2}(q_2-q_1)^\alpha\int{d^4s\over (2\pi)^4}[\partial_\alpha
W_{\nu\gamma}(s)+\ldots]
\end{equation}
where the higher order terms, denoted by the ellipses, vanish, while
the piece we have retained can be evaluated via Gauss' theorem, yielding
\begin{equation}
q_1^\mu T_{\mu\nu\gamma}(q_1,q_2)={-ie^2\over
8\pi^2}\epsilon_{\mu\nu\gamma\delta}q_1^\mu q_2^\delta\label{eq:fds}
\end{equation}
Similarly we find
\begin{equation}
q_2^\nu T_{\mu\nu\gamma}(q_1,q_2)={ie^2\over
8\pi^2}\epsilon_{\mu\nu\gamma\delta}q_1^\mu q_2^\delta\label{eq:fdt}
\end{equation}
and
\begin{equation}
(q_1+q_2)^\gamma T_{\mu\nu\gamma}(q_1,q_2)=0
\end{equation}
From Eqs. \ref{eq:fds} and \ref{eq:fdt} then we observe that electromagnetic gauge invariance
is violated, which would have serious
consequences for photon interactions.  This problem can be solved by
appending a polynomial in the external momenta, which can be done
without affecting the absorptive component of the amplitude.  Thus
defining the physical decay amplitude via
\begin{equation}
t^{phys}_{\mu\nu\gamma}(q_1,q_2)=T_{\mu\nu\gamma}(q_1,q_2)-{ie^2\over
8\pi^2}\epsilon_{\mu\nu\gamma\delta}(q_1-q_2)^\delta
\end{equation}
we see that gauge invariance is restored
\begin{equation}
q_1^\mu t^{phys}_{\mu\nu\gamma}(q_1,q_2)=q_2^\nu
t^{phys}_{\mu\nu\gamma}(q_1,q_2)=0
\end{equation}
However, taking the axial current divergence now yields
\begin{equation}
(q_1+q_2)^\gamma t^{phys}_{\mu\nu\gamma}(q_1,q_2)={ie^2\over
4\pi^2}\epsilon_{\mu\nu\gamma\delta}q_1^\gamma q_2^\delta
\end{equation}
so that the axial current is no longer conserved.  Thus, the axial
symmetry has been {\it broken} via a proper quantization of the
theory---there exists an anomaly.  We have then
\begin{equation}
t^{phys}_{\mu\nu\gamma}(q_1,q_2)={q_{1\gamma}+q_{2\gamma}\over
(q_1+q_2)^2+i\epsilon}{ie^2\over 4\pi^2}\epsilon_
{\mu\nu\alpha\beta}q_1^\alpha q_2^\beta
\end{equation}
which corresponds to the operator condition
\begin{equation}
\partial^\mu J^3_{5\mu}={e^2\over
16\pi^2}F_{\mu\nu}\tilde{F}^{\mu\nu}
\end{equation}
Using the PCAC condition, we have then
\begin{equation}
<2\gamma|\partial^\mu J^3_{5\mu}|0>=F_\pi m_\pi^2 {1\over
m_\pi^2}<2\gamma|\pi^0>={e^2\over
4\pi^2}\epsilon_{\mu\nu\alpha\beta}q_1^\mu \epsilon_1^\nu q_2^\alpha
\epsilon_2^\beta
\end{equation}

Since this evaluation represents a simple (LO) perturbative
calculation, one should ask about the influence of
interactions, whether these are from higher order electromagnetic or
strong interactions. The answer, as shown by Adler and
Bardeen\cite{adb}, is that such effects do {\it not} modify the
chiral anomaly. The basic argument is that any such interactions
will result in changes to the triangle diagrams in which the linear
divergence is removed---the diagrams become more convergent. Because
of this modification the vanishing of Eq. \ref {eq:dg} from such
diagrams is assured and we conclude that the lowest order
calculation given above must be true to {\it all} orders.

\subsection{Alternative Approaches:  All Roads Lead to Rome}

What are some of the alternative methods that can be used in order
to deal with the short distance behavior?  Some of the possibilities
include:

\begin{itemize}

\item [i)] Pauli-Villars Regularization:  As has already been mentioned, a Pauli-Villars regulator
can be used in order to make the results finite.  In this procedure
one defines the physical amplitude as the difference of the
amplitude calculated as above and the same amplitude calculated with
quarks having large mass $M$, {\it i.e.},
\begin{equation}
T^{physical}_{\mu\nu\lambda}(q_1,q_2)=\lim_{M\rightarrow\infty}
\left[T_{\mu\nu\lambda}(q_1,q_2)-T^M_{\mu\nu\lambda}(q_1,q_2)\right]
\end{equation}
where $T^M_{\mu\nu\lambda}(q_1,q_2)$ is identical to
$T_{\mu\nu\lambda}(q_1,q_2)$ but with the massless fermion
propagators replaced by propagators having mass $M$, {\it i.e.},
\begin{equation}
T^M_{\mu\nu\gamma}(q_1,q_2)=U^M_{\mu\nu\gamma}(q_1,q_2)+U^M_{\nu\mu\gamma}(q_2,q_1)
\end{equation}
where
\begin{eqnarray}
U^M_{\mu\nu\gamma}(q_1,q_2)&=&-{ie^2\over 2}K_F\int{d^4s\over
(2\pi)^4}\nonumber\\
&\times&{\rm Tr}\left({1\over
\not\!{s}+\not\!{q}_1-M}\gamma_\mu{1\over
\not\!{s}-M}\gamma_\nu{1\over
\not\!{s}-\not\!{q}_2-M}\gamma_\gamma\gamma_5\right)
\end{eqnarray}
Taking the axial divergence we find
\begin{equation}
(q_1+q_2)^\lambda U^M_{\mu\nu\lambda}(q_1,q_2)={e^2\over
16\pi^2}K_F\epsilon_{\mu\nu\alpha\beta}q_1^\alpha q_2^\beta
\end{equation}
so that
\begin{equation}
(q_1+q_2)^\lambda T^{physical}_{\mu\nu\lambda}(q_1,q_2)={e^2\over
4\pi^2}K_F\epsilon_{\mu\nu\alpha\beta}q_1^\alpha q_2^\beta
\end{equation}
We reproduce in this way then the axial anomaly
\begin{equation}
\partial^\lambda J^3_{5\lambda}={e^2\over 16\pi^2}F_{\mu\nu}\tilde{F}^{\mu\nu}
\end{equation}



\item [ii)] Path Integration: Path integral methods can also be
used.  In this case one quantizes by using the generating
functional, which sums over all field configurations
\begin{equation}
W=\int[d\psi][d\bar{\psi}][dA_\mu]\exp iS[\psi,\bar{\psi}, A_\mu]
\end{equation}
Now if we alter the field transformation Eq. \ref{eq:ku} or
Eq. \ref{eq:jn} from a {\it global} to a {\it local one} the action becomes
\begin{equation}
S[\psi',\bar{\psi}', A_\mu]=S[\psi,\bar{\psi}, A_\mu]+\int
d^4x\beta(x)\partial^\mu J_\mu(x)
\end{equation}
(Note that by using a local rather than a global field transformation
we are required to include a gauge boson field $A_\mu$ in addition to the
Dirac fields $\psi$ and $\bar{\psi}$.)
Kazuo Fujikawa showed that under a vector transformation---Eq.
\ref{eq:ku}---the integration measure is unchanged\cite{kfj}
\begin{equation}
%[d\psi'][d\bar{\psi}'][dA_\mu]=[d\psi_{V}'][d\bar{\psi_{V}'}][dA_\mu]
 [d{\psi'}_V][d{\bar{\psi}'}_V][dA_\mu]=[d\psi][d\bar{\psi}][dA_\mu]
\end{equation}
so that, requiring equality of the two representations for arbitrary
$\beta(x)$ yields
\begin{equation}
\partial^\mu J_\mu(x)=0
\end{equation}
{\it i.e.}, the classical field symmetry is also a quantum field
symmetry. However, this is {\it not} the case for a local axial
transformation---Eq. \ref{eq:jn}. In this case we have a non-unit
Jacobian
\begin{equation}
[d\psi_A'][d\bar{\psi}_A'][dA_\mu]=[d\psi][d\bar{\psi}][dA_\mu]J
\end{equation}
where
\begin{equation}
J=\exp(-2i{\rm Tr}\zeta(x) \gamma_5)
\end{equation}
Here the trace is over not only the Dirac indices but also over
spacetime and must be regulated in order not to diverge.  Employing
a covariant regulator of the form $$\exp(-\not\!\!{D}^2/M^2)$$ which
cuts off the high energy (short distance) modes, and the result
\begin{equation}
\not\!\!{D}^2=D^2+{eQ\over 2}\sigma_{\mu\nu}F^{\mu\nu}
\end{equation}
Fujikawa demonstrated that\cite{kfj}
\begin{equation}
J=\exp(-i\int d^4x \zeta(x){e^2\over
16\pi^2}F_{\mu\nu}\tilde{F}^{\mu\nu})
\end{equation}
The connection with the chiral anomaly can be made by noting that
the generating functional
\begin{equation}
W=\int[d\psi][d\bar{\psi}][dA_\mu]\exp iS[\psi,\bar{\psi}, A_\mu]
\end{equation}
after a local axial transformation Eq. \ref{eq:jn}, assumes the form
\begin{eqnarray}
W&=&\int[d\psi_{A}'][d\bar{\psi}_{A}'][dA_\mu]\nonumber\\
&\times&\exp i\left[S[\psi,\bar{\psi},
A_\mu]+\int d^4x \zeta(x)(\partial^\lambda
J^3_{5\lambda}(x)-{e^2\over
16\pi^2}F_{\mu\nu}\tilde{F}^{\mu\nu})\right]\nonumber\\
\quad
\end{eqnarray}
so that invariance of the functional integration for arbitrary
$\zeta(x)$ yields the anomaly condition
\begin{equation}
\partial^\lambda J^3_{5\lambda}={e^2\over 16\pi^2}F_{\mu\nu}\tilde{F}^{\mu\nu}
\end{equation}

\item[iii)] Point splitting:  Since the problems arise when the
field and its conjugate are at the same spacetime point, one can
define the axial current via the definition\cite{rjr}
\begin{equation}
J^3_{5\mu}(x)\equiv\lim_{\epsilon\rightarrow 0}\bar{\psi}(x+{1\over
2}\epsilon){1\over 2}\tau_3\gamma_\mu\gamma_5\psi(x-{1\over
2}\epsilon)\exp(ie\int_{x-{1\over 2}\epsilon}^{x+{1\over
2}\epsilon}dy_\beta A^\beta(y))
\end{equation}
If we now take the divergence we find
\begin{eqnarray}
i\partial^\mu J^3_{5\mu}(x)&=&\lim_{\epsilon\rightarrow
0}\left\{\bar{\psi}(x+{1\over 2}\epsilon){1\over
2}\tau_3\gamma_5\left[e\not\!\!{A}(x+{1\over
2}\epsilon)-e\not\!\!{A}(x-{1\over 2}\epsilon)\right]\psi(x-{1\over
2}\epsilon)\right.\nonumber\\
&-&\left.e\bar{\psi}(x+{1\over 2}\epsilon){1\over
2}\tau_3\gamma_\mu\gamma_5\psi(x-{1\over
2}\epsilon)\epsilon_\nu\partial^\mu
A^\nu\right\}\exp(ie\int_{x-{1\over 2}\epsilon}^{x+{1\over
2}\epsilon}dy_\beta A^\beta(y))\nonumber\\
&=&\lim_{\epsilon\rightarrow
0}e\epsilon_\nu\left\{\bar{\psi}(x+{1\over 2}\epsilon){1\over 2
}\tau_3\gamma_\mu\gamma_5\psi(x-{1\over
2}\epsilon)F^{\mu\nu}\exp(ie\int_{x-{1\over 2}\epsilon}^{x+{1\over
2}\epsilon}dy_\beta A^\beta(y))\right\}\nonumber\\
\quad
\end{eqnarray}
In taking the limit $\epsilon\rightarrow 0$ we use the short
distance behavior of the Dirac field\cite{rjr}
\begin{equation}
\lim_{\epsilon\rightarrow 0}{\rm Tr}\left[\epsilon_\nu{1\over
2}\tau_3\gamma_\mu\gamma_5<0|T\left(\psi(x-{1\over 2}\epsilon)\bar{\psi}(x+{1\over 2}
\epsilon)\right)|0>\right]={e\over 16\pi^2}\tilde{F}_{\mu\nu}
\end{equation}
to once again obtain the axial anomaly
\begin{equation}
\partial^\lambda J^3_{5\lambda}={e^2\over 16\pi^2}F^{\mu\nu}\tilde{F}_{\mu\nu}
\end{equation}

\item[iv)] Geometric Approach: Using geometric methods, Bardeen was
able to identify the full form of the anomaly\cite{wba}, which was soon thereafter
written in terms of an effective action by Wess and Zumino\cite{wzx}.  In the
case of SU(2) and electromagnetism the anomalous Lagrangian density
is
\begin{equation}
{\cal L}_A=-{N_c\over
48\pi^2}\epsilon^{\mu\nu\alpha\beta}\left[eA_\mu{\rm Tr}(QL_\nu
L_\alpha L_\beta-QR_\nu R_\alpha R_\beta)+ie^2F_{\mu\nu}A_\alpha
T_\beta\right]\label{eq:zx}
\end{equation}
where, defining
$$U=\exp(i\vec{\tau}\cdot\vec{\phi}_\pi/F_\pi),$$
\begin{eqnarray}
L_\mu&=&\partial_\mu UU^\dagger,\qquad R_\mu=\partial_\mu U^\dagger
U\nonumber\\
T_\beta&=&{\rm Tr}\left(Q^2L_\beta-Q^2R_\beta+{1\over 2}QUQU^\dagger
L_\beta-{1\over 2}QU^\dagger QUR_\beta\right)\label{eq:gx}
\end{eqnarray}
the piece of Eq. \ref{eq:zx} responsible for
$\pi^0\rightarrow\gamma\gamma$ can be found by expanding to first
order in the pion field
\begin{eqnarray}
{\cal L}_A&=&{e^2N_c\over 16\pi^2F_\pi}{\rm
Tr}(Q^2\tau_3)\epsilon^{\mu\nu\alpha\beta}F_{\mu\nu}A_\alpha\partial_\beta\pi^0\nonumber\\
&=&{e^2N_c\over 24\pi^2F_\pi}F_{\mu\nu}\tilde{F}^{\mu\nu}\pi^0
\end{eqnarray}
which once again reproduces the anomaly prediction.
\end{itemize}

In each case then, one is forced to modify short distance properties
in order to produce a consistent quantum field theory, and it is
this feature which breaks the classical symmetry and produces the
anomaly.  No matter how it is obtained, the result in the case of
the two photon decay amplitude of the neutral pion is that the decay
amplitude is precisely predicted to be
\begin{equation}
T_{\pi^0\gamma\gamma}={e^2\over 4\pi^2
F_\pi}\epsilon_{\mu\nu\alpha\beta}\epsilon_1^\mu\epsilon_2^\nu
q_1^\alpha q_2^\beta ,
\end{equation}
leading to a decay rate
\begin{equation}
\Gamma^{anom}_{\pi^0\gamma\gamma}={\alpha^2m_\pi^3\over
64\pi^3F_\pi^2}=7.76\,\,{\rm eV}\label{eq:lk}
\end{equation}
where $\alpha=e^2/4\pi$ is the fine structure constant, in good
agreement with the experimental value---{\it cf.} Fig. \ref{fig:width}.  However,
before a careful comparison of theory and experiment can be made, one must confront
the fact that the prediction Eq. \ref{eq:lk} is made in the limit of
chiral symmetry, rather than the real world.


\subsection{Real World Corrections}\label{sec:HO}

As mentioned above, the prediction Eq. \ref{eq:lk} is unsatisfactory
in that the chiral limit, in which both the $u,d$ quarks and the
pion are massless does not represent the real world. The $u,d$
quarks are light but not massless, and in turn the pion is the
lightest hadron but certainly does not possess zero mass. More
importantly, because the light quarks are nondegenerate, the
physical $\pi^0$ meson is {\it not} a pure U(3) state $|P_3>$ but is
instead a mixture of $|P_3>,\,|P_8>,\,$ and $|P_0>$ states.  This
mixing is important since a simple U(3) picture of the decay
predicts the bare amplitudes for the two photon decay to be
\begin{equation}
A_{P_3\gamma\gamma}:A_{P_8\gamma\gamma}:A_{P_0\gamma\gamma}=1:\sqrt{1\over
3}:2\sqrt{2\over 3}\label{eq:vx}
\end{equation}
so that, even if the mixture of $|P_8>,\,|P_0>$ states in the
neutral pion is small, they can play an important role in the
$\pi^0\rightarrow\gamma\gamma$ decay amplitude.  One should
note here that the predictions given in Eq. \ref{eq:vx} are given
via the use of U(3) symmetry, wherein the wavefunctions of the
$\eta_8$ and $\eta_0$ are taken to be identical.  This procedure is perhaps
somewhat surprising, since the $\eta_8$ is a Goldstone boson and is massless in the chiral
symmetric limit, while $\eta_0$ is not. The $\eta_0$ mass is known to arise
due to the axial singlet anomaly, but does vanish in the
$N_c\rightarrow\infty$ limit\cite{dgh}. Nevertheless, here and in
other circumstances the use of U(3) symmetry is known to give good
results\cite{nmc}. In terms of chiral perturbation theory, the
prediction of the chiral anomaly for the
$\pi^0\rightarrow\gamma\gamma$ decay amplitude, since it involves
the four-dimensional Levi-Civita tensor, is already
four-derivative--${\cal O}(q^4)$---and is two orders higher than the
leading order strong interaction chiral effects, which are ${\cal
O}(q^2)$\cite{chl}. (Note that we follow ref. \cite{uch} here in using the counting
${\cal O}(e)={\cal O}(q)$.) Modifications of the pion decay amplitude due to
particle mixing are also ${\cal O}(q^4)$. Since the pion is an isovector
while the $\eta$ and $\eta^{'}$ are isoscalars the associated mixing matrix elements must be proportional to
$${m_u-m_d}.$$  (Of course, there exist in addition corrections of ${\cal
O}(q^6)$ which involve factors such as $m_\pi^2/\Lambda_\chi^2$, but
these are presumably higher order and somewhat smaller than those which come
from mixing.)

It is useful to make a simple back of the envelope calculation of
the modifications due to mixing effects by use of the representation
of the physical states $|\pi^{0},\eta,\eta^{'}>$ in terms of the bare U(3) states
P = $|\pi_{3},\eta_{8}, \eta_{0}>$. In order to do this it is useful to first review
the $P \rightarrow \gamma \gamma$ decay rates predicted by the anomaly
\begin{eqnarray}
A_{P \gamma\gamma}&=&{e^2\over 16\pi^2F_P} \\ \nonumber
\Gamma_{\pi\gamma\gamma}&=&{|A_{\pi\gamma\gamma}|^2 m_P^3\over 4\pi}
\label{eq:Gamma-P}
\end{eqnarray}
where $m_P, F_P$ represents the mass, decay constants of the respective pseudoscalars.
In Eq. \ref{eq:vx} the relative amplitudes were given in lowest order, where all of
the decay constants are equal. In the next chiral order there are corrections
to this equality\cite{Donoghue:1985} which lead to $F_{8}/F_{3} = F_{\eta}/F_{\pi} \simeq$ 1.25 and
$F_{0}/F_{3} = F_{\eta^{'}}/F_{\pi} \simeq$ 1.  We shall use these modified values to amend
Eq. \ref{eq:vx}.  With this adjustment, the two-gamma widths are calculated to be
$\Gamma (\eta \rightarrow \gamma \gamma)$ = 0.11 keV and $\Gamma (\eta^{'} \rightarrow \gamma \gamma)$
= 7.40 keV and are {\it not} in agreement with the experimental results
$\Gamma (\eta \rightarrow \gamma \gamma) \simeq ( 0.51 \pm 0.05)$ keV and
$\Gamma (\eta^{'} \rightarrow \gamma \gamma) \simeq 4.28 \pm 0.38$ keV\cite{PDB}.
The fact that the calculated width of the $\eta$ is too low, while that of the $\eta^{'}$ is too high,
is strong evidence for $\eta, \eta^{'}$ mixing, which one can introduce by writing\cite{Donoghue:1985}
\begin{eqnarray}
|\eta>  &=& \cos\theta|\eta_{8}> - \sin\theta |\eta_{0}> \\ \nonumber
|\eta^{'}>  &=& \sin\theta |\eta_{8}> + \cos\theta|\eta_{0}>
\label{eq:theta}
\end{eqnarray}
Using this representation one obtains for the decay amplitudes
\begin{eqnarray}
A_{\eta \gamma\gamma}  &=& \frac{\alpha}{4 \pi \sqrt{3}} ~\Bigg{[ }\frac{ \cos\theta}{ F_{\eta} }- \frac{\sin\theta \sqrt{8} }{ F_{\eta^{'}}}~\Bigg]\\ \nonumber
A_{\eta^{'} \gamma\gamma}  &=& \frac{\alpha}{4 \pi \sqrt{3}} ~\Bigg{[ }\frac{ \sin\theta}{ F_{\eta} } +\frac{\cos\theta \sqrt{8} }{ F_{\eta^{'}}}~\Bigg]
\label{eq:mixing}
\end{eqnarray}
and, treating $\theta$ as a free parameter, one can obtain agreement with the experimental values\cite{PDB} by using $-25\, {\rm deg}\leq \theta\leq -20 \,{\rm deg}$\cite{Donoghue:1985}.

There exists another method to estimate this mixing, which is instructive and will be helpful in estimating the chiral corrections to the $\pi^0$ decay rate.  One simply diagonalizes the mass matrix to obtain the physical $\eta, \eta^{'}$ states and the mixing angle
\begin{equation}
\left(
\begin{array} {cc}
m_{8}^{2} -M^{2} & m_{08}^{2} \\
m_{08}^{2} & m_{0}^{2} -M^{2}
\end{array}
\right )
 \left(
\begin{array} {c}
|\eta>\\
|\eta^{'}>
\end{array}
\right)
~ = ~0
\label{eq:matrix}
\end{equation}
where $m_{8}, m_{0}, m_{08}$, represent the masses of the unperturbed $\eta_{8},\eta_{0}$ states and the off-diagonal mass mixing matrix element, which we take as a parameter.  (The eigenvalue equation involves the square of the masses since $\eta ,\eta'$ are bosons.) There exist two eigenvalues for ${\cal M}$ which are $m^2_{\eta}, m^2_{\eta^{'}}$.  To solve this eigenvalue equation we need the value of $m_{8}$ which can be obtained from the relationship
\begin{eqnarray}
m_{8}^{2}  &=& \frac{1}{3} (4 m_{K}^{2} -m_{\pi}^2) (1+ \delta) \\ \nonumber
m_{K}^{2} &=& \frac{1}{2} (m_{K^0}^{2} + m_{K^{+}}^{2})
\label{eq:GMO}
\end{eqnarray}
For $\delta$ = 0 Eq. 77 is simply the Gell-Mann-Okubu mass formula
\begin{equation}
4m_K^2=3m_\eta^2+m_\pi^2,\label{eq:bz}
\end{equation}
which is derived via the use of SU(3) symmetry.  Since SU(3) is not exact, there exist chiral corrections, for which a leading-log estimate gives $\delta \simeq$ 0.16\cite{Donoghue:1985}. The value of $m_{0}$ can be obtained by observing that, from the trace of the mass matrix in  Eq. \ref{eq:matrix} we have $m_{8}^{2} + m_{0}^{2} = m_{\eta}^{2} + m_{\eta^{'}}^{2}$. Taking $\delta$ as a free parameter, the eigenvectors (specified by the angle $\theta$ of Eq. \ref{eq:theta})  can be obtained and from this the decay rates $\Gamma(\eta, \eta^{'} \rightarrow \gamma, \gamma)$, yielding $0.16\leq\delta\leq 0.22$ in approximate agreement with the leading-log estimate\cite{Donoghue:1985}.

Now we are ready to estimate the magnitude of $\eta, \eta^{'}$ mixing in the $\pi^{0}$ amplitude, which can be approximately written as
\begin{eqnarray}
|\pi^{0} > \simeq | \pi_{3}> + \theta_{\eta} |\eta> + \theta_{\eta^{'}} |\eta^{'}>
\label{eq:pi0-mixing}
\end{eqnarray}
since the mixing angles are small.  The mixing amplitudes $\theta_{\eta}, \theta_{\eta^{'}}$ can be obtained using perturbation theory. The off diagonal matrix elements of the mass matrix $M$ (see, {\it e.g.}, ref. \cite{dgh}) and the mass matrix mixing amplitudes in terms of the quark masses are
\begin{eqnarray}
m_{38}^{2}  &=& < \eta_{8} | M | \pi_{3}> = \frac{B_{0}}{\sqrt{3}} (m_{d} - m_{u})\nonumber \\
m_{30}^{2} &=&  < \eta_{0} | M | \pi_{3}> = \frac{\sqrt{2} B_{0}}{\sqrt{3}} (m_{d} - m_{u})
\nonumber \\
\theta_{\eta} &=& \frac{\cos\theta m_{38}^{2} - \sin\theta m_{30}^{2}}{m_{\eta}^{2} - m_{\pi^{0}}^{2}} \nonumber \\
\theta_{\eta^{'}} &=& \frac{\sin\theta m_{38}^{2} + \cos\theta m_{30}^{2}}
{m_{\eta^{'}}^{2} - m_{\pi^{0}}^{2}}
\label{eq: pi-mixing}
\end{eqnarray}
where $B_0$ is related to the vacuum expectation value of the
quark scalar density via
\begin{equation}
B_0=-{1\over F_0^2}<0|\bar{q}q|0>\simeq {m_\pi^2\over 2\hat{m}}
\label{eq:B0}
\end{equation}
Using the value of $B_{0}$ in terms of $m_{\pi^{0}}$ and the quark mass ratio $m_{u}/m_{d} \simeq 0.56$\cite{Leutwyler:2009} numerical calculations can be performed.  A number of interesting features emerge. First the decay rate is increased  by $\simeq$ 4\%. This value is only weakly dependent on the parameter $\delta$ which corrects the Gell-Mann-Okubo mass formula Eq. \ref{eq:bz}. For $\delta \simeq$ 0.18, for which the $\eta,\eta^{'}$ rates are in agreement with experiment, the values of
$\theta_{\eta} \simeq$ 0.015 rad and $\theta_{\eta^{'}} \simeq$ 0.0032 rad are obtained. The resultant value of $\Gamma(\pi^{0} \rightarrow \gamma \gamma) \simeq $8.1 eV represents a $\simeq$ 4.5\% increase over the value predicted by the chiral anomaly. The contribution of the $\eta$ is
$\simeq$ 3 \% while from the $\eta^{'} \simeq$ 1\%. As we shall see, it is remarkable that this back of the envelope estimate is
in good agreement with various careful chiral perturbation theory calculations.

Stimulated by the PrimEx experiment, QCD corrections to the chiral anomaly prediction
for the $\pi^0\rightarrow\gamma\gamma$ decay amplitude were estimated by a number of groups
with remarkably similar results.  As mentioned above, the leading order (LO) anomaly amplitude already involves four derivations and
is ${\cal O}(q^4)$, while higher order (HO) corrections have been estimated within various approximation schemes.  (It is because
"higher order" means different things depending on the calculation that we have chosen to use this notation, rather than the usual NLO.)
\begin{itemize}

\item [a)] A sum rule estimate by Ioffe and Oganesian\cite{ioo}
including {\it only} $\pi^0,\,\eta^0$ mixing yielded a 3\%
enhancement---$\Gamma_{\pi^0\rightarrow\gamma\gamma}=7.93\pm 0.12$
eV.  The fact that this result is nearly 2{\%} lower than the other three studies can be understood by the omission of
the $\eta -\eta'$ mixing effect given above.
\end{itemize}

\noindent Other authors {\it have} included mixing with the $\eta'$ within the
context of various approximations to QCD:

\begin{itemize}

\item [b)] The work of Goity, Bernstein, and Holstein\cite{bgh} involves
the use of chiral $U(3)\times U(3)$ symmetry and the large $N_c$
limit in order to include the $\eta'$ as a Goldstone boson and
includes modifications to the anomaly prediction of ${\cal
O}(q^6)$ and ${\cal O}(q^4\times {1\over N_c})$.  Such corrections
predict a 4.5\% enhancement to the decay
rate---$\Gamma_{\pi^0\rightarrow\gamma\gamma}=8.13\pm 0.08$ eV.

\item [c)] An alternate approach was taken by Ananthanarayan and
Moussallam\cite{anm}, who employed chiral perturbation theory in the
anomaly sector with the inclusion of dynamical photons.  In this way
they looked both at quark mass effects and at electromagnetic
corrections of ${\cal O}(q^6)$.  The result was a predicted decay
rate---$\Gamma_{\pi^0\rightarrow\gamma\gamma}=8.06\pm 0.02\pm 0.06$
eV, in excellent agreement with the Goity et al. calculation.

\item [d)] The work of Kampf and Moussallam\cite{kam}
involved an NNLO calculation within two flavor chiral perturbation theory.  However,
there exist a number of undetermined counterterms which were estimated by use of a modified
counting scheme wherein $m_s$ is taken to be of ${\cal O}(q)$. The
result was a prediction---$\Gamma_{\pi^0\rightarrow\gamma\gamma}=8.09\pm 0.11$
eV.
\end{itemize}

These values are plotted in Fig. \ref{fig:Gamma-ChPT2}.
There is obviously little scatter among these theoretical
calculations which assert that chiral symmetry breaking quark mass effects
increase the decay rate of the neutral pion from its $7.76$ eV value
predicted by the anomaly to  8.10 eV, the average of these results.  The basic
reason responsible for this 4.5\% enhancement can be found in the
pseudoscalar mixing estimate given above.   On the theoretical side, the possible
$\sim 1$\% errors in the $\pi^0\gamma\gamma$ decay rate estimates arise not from
convergence issues in the chiral expansion but rather from uncertainty in some of the calculational
input parameters as well as the mixing estimates due to isospin breaking.
Since these predictions are already at the one loop level in the chiral %/N_
expansion, it is unlikely that they will be significantly improved in the near future.
However, in order to confirm this enhancement it is clearly necessary to perform an
experiment looking at $\pi^0\rightarrow\gamma\gamma$ decay at the percent level.

\begin{figure}
\begin{center}
\includegraphics*[width=1\linewidth,clip=true]{Gamma-ChPT2.pdf}
\end{center}
\vspace{-4cm}
\caption{The $\Gamma(\pi^{0} \rightarrow \gamma \gamma)$ width in eV predicted by the NLO chiral calculations, GBH\cite{bgh}, AM\cite{anm}, and KM\cite{kam}. The lower dashed line is  the predictions of the LO chiral anomaly\cite{bej,sdl} ($\Gamma(\pi^{0} \rightarrow \gamma \gamma) = 7.760\,\,{\rm eV}, \tau(\pi^{0}) = 0.838\times 10^{-16}$ s.). The upper solid line is  the average value of the NLO chiral prediction and the dotted lines show the estimated 1\% error ($\Gamma(\pi^{0} \rightarrow \gamma \gamma)= 8.10\,\,{\rm eV}, \tau(\pi^{0})= 0.80\times 10^{-16}$ s.).
\label{fig:Gamma-ChPT2}}
\end{figure}


\subsection{Other Anomalous Processes}\label{sec:Other}

From the form of the full SU(2) anomalous effective Lagrangian Eq.
\ref{eq:zx}, it is clear that, in addition to the triangle diagrams
which we have considered above, there also exist anomalous box and
pentagon diagrams.  The presence of the Levi-Civita tensor means
that the processes described by Eq. \ref{eq:zx} are of a different
character than those described by the conventional chiral
Lagrangian\cite{chl}.  Witten\cite{wit} has pointed out that under
what he calls an "intrinsic parity transformation" under wherein pseudoscalar fields undergo a change of sign
but spacetime coordinates remain unchanged
$$\phi^P\rightarrow -\phi^P\quad {\rm so}\quad U=\exp({i\over F_P}\sum_{j=1}^8\lambda_j\phi_j^P)\rightarrow
\exp({-i\over F_P}\sum_{j=1}^8\lambda_j\phi_j^P)=U^\dagger ,$$
the conventional chiral Lagrangian ala Gasser and Leutwyler\cite{chl},\cite{chl1}, which contains terms
such as
$${\rm Tr}\partial_\mu U^\dagger\partial^\mu U,\,\,[{\rm Tr}\partial_\mu U^\dagger\partial^\mu U]^2,\,\,
{\rm Tr}(\partial_\mu U^\dagger\partial_\nu U){\rm Tr}(\partial^\mu U^\dagger\partial^\nu U),\,\, etc.,
$$
includes only the interactions of an {\it even} number of pseudoscalars (or
axial currents) or the coupling of one or two photons to two, four,
six, {\it etc.} pseudoscalars or axial currents, while the SU(2) anomalous Lagrangian
of Eq. \ref{eq:zx} (and its SU(3) generalization) is antisymmetric under $U\rightarrow U^\dagger$ and $L_\mu\rightarrow R_\mu$
and so describes transitions between processes involving an {\it odd}
number of pseudoscalars (or axial currents) or of the coupling of
one or two photons to one, three, five, {\it etc.} pseudoscalars or axial
currents\cite{wit}.  The existence of the chiral anomaly then, in addition to predicting the decay
amplitude for $\pi^0\rightarrow\gamma\gamma$, also makes {\it parameter-free} predictions for processes such as
\begin{itemize}
\item[a)] $\gamma\pi^0\rightarrow\pi^+\pi^-$
\item[b)] $\pi^+\rightarrow e^+\nu_e\gamma$
\item[c)] {\it etc}.
\end{itemize}

or, by extending our analysis to the case of SU(3), for reactions
such as
\begin{itemize}
\item[d)] $K^+K^-\rightarrow\pi^+\pi^-\pi^0$
\item[e)] $\eta\rightarrow\pi^+\pi^-\gamma$
\item[f)] $K^+\rightarrow\pi^+\pi^-e^+\nu_e$
\item[g)] $K^+\rightarrow e^+\nu_e\gamma$
\item[h)] {\it etc.}
\end{itemize}

Note here that when a weak interaction is involved, the coupling to the lepton pair $e^+\nu_e$ is associated
with both a polar vector as well as an axial vector current.  The axial current behaves like a pseudoscalar
under an intrinsic parity transformation so that, for example, the process $\pi^+\rightarrow e^+\nu_e\gamma$
has even intrinsic parity when mediated by the axial current and is not anomalous.  However, if the leptons
couple via a polar vector current, the same process has odd intrinsic parity and occurs via the anomaly.

While it is possible in principle to probe the validity of the chiral anomaly by measurements of any
these reactions, analysis of the $K_{\ell 4}$ decay (f) generally {\it assumes} the value for the appropriate vector form factor predicted by the anomaly.  In the radiative $\eta$ decay reaction (e), significant mixing
with the $\eta'$ obscures a precise test of the chiral anomaly\cite{vgp}.  In the case of the $\gamma 3\pi$
vertex (a) a test was performed many years ago by Antipov et al. with the result\cite{atv},\cite{atw}
\begin{equation}
{\rm Amp}_{\gamma 3\pi}^{exp}=(12.9\pm 0.9\pm 0.5)\,{\rm GeV}^3\quad{\rm vs.}\quad
 {\rm Amp}_{\gamma 3\pi}^{anomaly}={eN_c\over 12\pi^2 F_\pi^3}=9.7\,{\rm GeV}^3
\end{equation}
However, comparison of theoretical and experimental results is not as straightforward as in the case of neutral pion decay.  Of course, "real world" chiral symmetry breaking and electromagnetic corrections similar to those calculated in the case of the $\pi^0\rightarrow\gamma\gamma$ decay amplitude affect ${\rm Amp}_{\gamma 3\pi}^{anomaly}$ and must be included\cite{rhc}.  But also, the reaction  $\gamma\pi^0\rightarrow \pi^+\pi^-$ has an energy dependence that must be accounted for in comparing with the anomaly prediction\cite{khb}, which is calculated in the chiral limit.  Certainly, an up to date modern measurement of the $\gamma 3\pi$ amplitude would be of interest.

Another reaction that has been utilized as a test of the chiral anomaly is radiative pion decay (b).  Since this process is used by the PDG in their determination of the neutral pion decay lifetime, it will be discussed next in more detail.  However, while examination of any of the reactions listed above and their connection to the chiral anomaly is of interest, in the present paper, we shall focus on the $\pi^0\rightarrow\gamma\gamma$ process.

\subsection{Radiative Pion Beta Decay}\label{sec:pi-beta}
The PIBETA experiment mentioned in the introduction uses a {\it measured} weak polar vector form factor to predict the neutral pion decay amplitude by isospin invariance and is used as an input to the PDG average\cite{Bychkov:2009}.  Because of this, we here discuss this process in a bit more detail.  The transition amplitude can be written in general as
\begin{equation}
{\cal M}_{\pi^+\rightarrow e^+\nu_e\gamma}=-{eG_F\over \sqrt{2}}V_{ud}M_{\mu\nu}(p,q)
\epsilon^{\mu *}\bar{u}(p_\nu)\gamma^\nu(1+\gamma_5)v(p_e)
\end{equation}
where $G_F$ is the weak decay constant, $V_{ud}$ is the CKM parameter connecting the $u$ and $d$ quarks, and\cite{dgh}
\begin{eqnarray}
M_{\mu\nu}(p,q)&=&\int d^4xe^{iq\cdot x}<0|T(J_\mu^{em}(x)J_\nu^{1-i2}(0)|\pi^+(p)>\nonumber\\
&=&-\sqrt{2}F_\pi{(p-q)_\nu\over (p-q)^2-m_\pi^2})<\pi^+(p-q)|J_\mu^{em}|\pi^+(p)>+\sqrt{2}F_\pi g_{\mu\nu}\nonumber\\
&-&{1\over m_\pi}F_A((p-q)_\mu q_\nu-g_{\mu\nu}q\cdot(p-q)) + i {1\over m_\pi}F_V\epsilon_{\mu\nu\alpha\beta}q^\alpha p^\beta\label{eq:bg}
\end{eqnarray}
Here the second line represents the Born diagram together with a contact term required for gauge invariance and in the following line the subscripts $V$ and $A$ indicate whether the weak vector or axial-vector of the weak currents are involved.  The purpose of the PIBETA experiment was to measure the rate of the pion beta decay reaction $\pi^+\rightarrow \pi^0e^+\nu_e$ as a test of the conserved vector current (CVC) relation or, by using CVC, to measure the CKM parameter $V_{ud}$ in a reaction where strong interaction uncertainties are not important.  Because this is such a small ($\sim 10^{-8}$) branching ratio process, the experiment also detected other higher branching ratio reactions such as radiative pion decay $\pi^+\rightarrow e^++\nu_e+\gamma$.  Ordinarily a radiative decay is primarily sensitive to the Born amplitude, which simply generates a correction to the non-radiative decay process via
\begin{equation}
{d\Gamma\over d\Omega dk}\sim {\alpha\over k}{d\Gamma_0\over d\Omega}+\ldots
\end{equation}
so that direct decay amplitudes are hidden under this huge bremsstrahlung background.  However, because the nonradiative decay process $\pi^+\rightarrow e^+\nu_e$ is helicity-suppressed the direct decay amplitudes $h_V,\,h_A$
above can both be measured and this was done by the PIBETA experimenters.  The direct axial-vector decay amplitude $F_A$ determines, via PCAC, the charged pion polarizability\cite{gxr}, while the direct polar-vector amplitude $F_V$ is related to the pion decay constant via\cite{dgh}
\begin{equation}
A_{\pi^0\gamma\gamma}={e^2\over 2\sqrt{2}m_\pi}F_V\label{eq:lz}
%\label{eq:bt}
\end{equation}
That this should be the case is clear from the Wess-Zumino anomaly Lagrangian Eq. \ref{eq:zx} or simply from isotopic spin invariance.  Indeed since the pion as well as the isoscalar component of the electromagnetic current have negative G-parity while the isovector piece of the electromagnetic current has positive G-parity, the two-photon decay of the $\pi^0$ must involve both isoscalar and isovector pieces of $J_\mu^{em}$, so
\begin{equation}
2A_{\pi\gamma\gamma}\epsilon_{\mu\nu\alpha\beta}q^\alpha(p-q)^\beta=e^2\int d^4xe^{iq_1\cdot x}<0|T(^{I=0}J_\mu^{em}(x)^{I=1}J_\nu^{em}(0))|\pi^0(\vec{p})>
\end{equation}
G-invariance also requires the direct polar vector radiative pion decay amplitude $F_V$ to involve only the isoscalar component of the electromagnetic current
\begin{equation}
{1\over m_\pi}F_V\epsilon_{\mu\nu\alpha\beta}q^\mu(p-q)^\nu=\int d^4xe^{iq_1\cdot x}<0|T(^{I=0}J_\mu^{em}(x)^{1-i2}J_\nu(0))|\pi^0(\vec{p})>
\end{equation}
By CVC these two transition amplitudes are related via
\begin{eqnarray}
\int d^4xe^{iq_1\cdot x}<0|T(^{I=0}J_\mu^{em}(x)^{I=1}J_\nu^{em}(0))|\pi^0(\vec{p})>\nonumber\\
=\sqrt{1\over 2}\int d^4xe^{iq_1\cdot x}<0|T(^{I=0}J_\mu^{em}(x)^{1-i2}J_\nu(0))|\pi^0(\vec{p})>
\end{eqnarray}
from which Eq. \ref{eq:lz} follows.  Thus a measurement of $F_V$ can be used to yield an experimental value for the $\pi^0\rightarrow\gamma\gamma$ decay rate
\begin{equation}
\Gamma_{\pi\gamma\gamma}={1\over 2}\pi m_\pi\alpha^2|F_V|^2
\end{equation}
The result of the PIBETA experiment gives\cite{Bychkov:2009}
\begin{equation}
\Gamma_{\pi^0\gamma\gamma}^{\rm pi-beta}=7.7\pm 1.0 \,{\rm eV},\label{eq:zj}
\end{equation}
and this number is included in the PDG average.

Note, however, that since isospin invariance is broken at the $\sim$1\% level, the present 11\% precision of this method is not an issue, but the uncertainty associated with isospin violation ultimately limits its use at the $\sim$1\% level unless this breaking is included.  The breaking associated with the neutral pion decay amplitude was discussed in the previous section and amounts to a $\simeq$ 2.3\% increase in the decay amplitude.  However, we also need to know the isospin violation---both from electromagnetic corrections as well as from the u-d quark mass difference---in the radiative pion decay amplitude.  These breaking effects have been calculated by Unterdorfer and Pichel\cite{unp} and were included in the PIBETA\cite{Bychkov:2009} analysis except for a $\simeq$ 0.9\% increase to the radiative pion decay vector form factor $F_V$.  Thus the proper way in which to determine the neutral pion decay amplitude from the experimental value of $F_V$ is to increase the CVC-predicted value of the neutral pion decay amplitude---Eq. \ref{eq:lz}---by 2.3-0.9\%=1.4\%, so that the pion decay rate predicted in Eq. \ref{eq:zj} becomes $7.9\pm 1.0$ eV.  Since the uncertainty in the PIBETA\cite{Bychkov:2009} value of $F_V$ is at the 11\% level, this modification is not important at the present time, but could be a factor in a future precision determination.


\subsection{Physics of the Anomaly}

Above we have shown how the chiral anomaly leads to a remarkable
successful agreement between experiment and theory for the decay
rate of the neutral pion.  However, this derivation is somewhat
formal and it remains to show what the "physics" of the anomaly
is---that is, {\it why} must quantization destroy the classical
axial symmetry.  In order to present an answer to this question it
is useful to first examine the Schwinger model, which is the name
generally given to massless electrodynamics in one plus one
dimensions\cite{jsc}.  Here the Lagrange density is given by
\begin{equation}
{\cal L}=\bar{\psi}i\not\!\!{D}\psi-{1\over 4}F_{\mu\nu}F^{\mu\nu}
\end{equation}
where
\begin{equation}
D_\mu=\partial_\mu+ieA_\mu
\end{equation}
is the covariant derivative and the $2\times 2$ Dirac matrices are
given in terms of the Pauli matrices via
\begin{equation}
\gamma^0=\sigma_1\quad{\rm and}\quad\gamma^1=i\sigma_2
\end{equation}
It is then easy to see at the classical level that we have equations
of motion
\begin{equation}
i\not\!\!{D}\psi=0\quad{\rm and}\quad\Box A_\mu=ej_\mu\label{eq:vc}
\end{equation}
where
\begin{equation}
j_\mu=\bar{\psi}\gamma_\mu\psi
\end{equation}
is the vector current and is conserved---$\partial^\mu j_\mu=0$. There also exists an axial current
\begin{equation}
j_\mu^5=\bar{\psi}\gamma_\mu\gamma_5\psi\quad{\rm with}\quad
\gamma_5=-\gamma^0\gamma^1=\sigma_3
\end{equation}
which is conserved---$\partial^\mu j_\mu^5=0$.  For later use, we
note also that
\begin{equation}
j_\mu^5=\epsilon_{\mu\nu}j^\nu\label{eq:hb}
\end{equation}
where $\epsilon_{\mu\nu}$ is the two-dimensional Levi-Civita tensor.
So far then, this looks simply like a two-dimensional version of
massless QED.

However, upon quantization it can be shown that the Lagrangian can
be written as
\begin{equation}
{\cal L}=\bar{\psi}'i\not\!{\partial}\psi'-{1\over
4}F_{\mu\nu}F^{\mu\nu}-{e^2\over 2\pi}A_\mu A^\mu
\end{equation}
that is, in terms of a noninteracting system of massless spin 1/2
particles and free "photons" having mass $m^2_\gamma=e^2/\pi$.  Also
in the quantized theory the axial current is no longer conserved.
Rather we have
\begin{equation}
\partial^\mu j_\mu^5=-{e\over 2\pi}\epsilon^{\mu\nu}F_{\mu\nu}
\end{equation}
That is, axial current conservation is broken by
quantization---there exists an anomaly.

The physical origin of the anomaly can be seen via an argument due
to Widom and Srivastava\cite{srw} by considering the vacuum state in
the quantized theory, which, according to Dirac, can be considered
as a filled set of negative energy states.  In the absence of an
external electric field there exists a density of electron states
$dp/2\pi$ with momenta evenly distributed between $p=-\infty$ and
$p=\infty$, and so there is no net current.  Now consider what
happens in the presence of a constant electric field $E$---a net
current flow develops, which increases with time. In terms of the
current density $j$ we have
\begin{equation}
{dj\over dt}=e\int_{-\infty}^\infty {dp\over 2\pi}{dv\over dt}
\end{equation}
where, using the Lorentz force law---$dp/dt=eE$---we have
\begin{equation}
{dv\over dt}={d\over dt}{d\over dp}\sqrt{m^2+p^2}={eEm^2\over
(m^2+p^2)^{5\over 2}}
\end{equation}
Performing the integration we find a result
\begin{equation}
{dj\over dt}={e^2E\over \pi}
\end{equation}
which is {\it independent} of the mass.  Since the vacuum charge
density $\lambda$ is independent of position---$d\lambda/dx=0$---we
have, defining $j^\mu=(\lambda,j)$ and using Eq. \ref{eq:hb}
\begin{equation}
e\partial^\mu j_\mu^5=-{e^2\over
2\pi}\epsilon^{\mu\nu}F_{\mu\nu}\label{eq:jg}
\end{equation}
which is the chiral anomaly.  Note that Eq. \ref{eq:jg} can also be
written as
\begin{equation}
0=\epsilon_{\mu\nu}\partial^\mu\left(ej^\nu+{e^2\over
\pi}A^\nu\right)
\end{equation}
In Lorentz gauge---$\partial^\mu j_\mu=0$---we have
\begin{equation}
j_\mu=-{e^2\over \pi}A_\mu
\end{equation}
so that the equation of motion in Eq. \ref{eq:vc} becomes
\begin{equation}
(\Box+{e^2\over \pi})A_\mu=0
\end{equation}
which indicates that the "photon" has developed a mass
$m^2_\gamma=e^2/\pi$.  We see then that in this picture the origin
of the anomaly is clear and arises from the feature that the vacuum
state of the quantized system is altered in the presence of an
applied electric field.

An alternative way to understand the same result has been given by
Jackiw\cite{rjk}, wherein one looks at solutions of the
time-independent Dirac equation
\begin{equation}
E\psi=\gamma_0\gamma_1\left(-i{\partial\over \partial
x}-eA\right)\psi
\end{equation}
In the case of a constant vector potential then there are two
classes of solutions
\begin{eqnarray}
\psi_+(x)&=&\left(\begin{array}{c} e^{ipx}\\0
\end{array}\right)\quad{\rm with}\quad E=p-eA\nonumber\\
\psi_-(x)&=&\left(\begin{array}{c}0\\e^{ipx}\end{array}\right)\quad{\rm
with}\quad E=-p+eA
\end{eqnarray}
where the subscript $\pm$ specifies the chirality of the
solution---{\it i.e.}, the eigenvalues of the operators ${1\over
2}(1\pm \gamma_5)$.  If $A=0$ we see then that the vacuum consists
of (negative energy) states with $p<0$ for positive chirality and
$p>0$ for negative chirality---{\it cf.} Fig. \ref{fig:theory3}.

\begin{figure}
\begin{center}
\includegraphics*[width=0.50\linewidth,clip=true]{Barry3.pdf}
\end{center}
\vspace{-5mm} \caption{The Dirac Sea in the case of a vanishing vector
potential.  Here a solid dot represents a filled state while an
empty dot signifies an empty state.
\label{fig:theory3}}
\end{figure}

Now suppose we make an adiabatic change from $A=0$ to a nonzero
field with $A=\epsilon$.  In the presence of the field, the vacuum
states become those with $p<e\epsilon$ for positive chirality and
$p>e\epsilon$ for negative chirality, meaning that there is a net
chirality production
\begin{equation}
\Delta\chi=2\int_0^{e\epsilon}{dp\over 2\pi}={e\epsilon\over
\pi}\label{eq:mz}
\end{equation}
This result should be expected from the chiral anomaly, which
requires a time-varying axial charge
\begin{equation}
{d\over dt}Q_5={e\over \pi}E={e\over \pi}{dA\over dt}\label{eq:bv}
\end{equation}
Since
\begin{equation}
Q_5=\int dx\psi^\dagger\sigma_3\psi
\end{equation}
corresponds to chiral charge, we find, integrating both sides of Eq.
\ref{eq:bv}
\begin{equation}
\Delta\chi={e\over \pi}\Delta A={e\epsilon\over \pi}
\end{equation}
in agreement with Eq. \ref{eq:mz}.  Once again we see that the
origin of the anomaly is the modification of the vacuum in the
presence of an applied electric field.

A simple handwaving argument can be used to generalize the latter
argument to four spacetime dimensions\cite{amu}.  A constant
magnetic field in the $z$-direction can be represented by the vector
potential
\begin{equation}
\vec{A}={1\over 2}\vec{B}\times\vec{r}
\end{equation}
The energies in the presence of the field are given by the Landau
levels
\begin{equation}
E_k=\pm\sqrt{p_z^2+2eBk}\quad{\rm with}\quad k=0,1,2,...
\end{equation}
If we now turn on an electric field, also in the
z-direction, then the energy levels change in accord with the
Lorentz force law
\begin{equation}
{d\vec{p}_z\over dt}=e\vec{E}
\end{equation}
As $p_z$ changes, the energy levels change, but negative energy
levels remain negative so that no particle creation occurs. However,
if $k=0$ then the structure of the levels is as in the case of the
Schwinger model, so that helicity is produced at the rate
\begin{equation}
{dh\over dt}=\rho{e\over 2\pi}E
\end{equation}
where $\rho$ is magnetic flux density.  Since magnetic flux density
is quantized in terms of $2\pi/e$, we have
\begin{equation}
\rho={eB\over 2\pi}
\end{equation}
and thus
\begin{equation}
{dh\over dt}={e^2\over 4\pi^2}EB
\end{equation}
Since helicity and chirality are the same for a massless system we
can write this as the covariant equation
\begin{equation}
{dQ_5\over dt}={e^2\over 4\pi^2}F_{\mu\nu}\tilde{F}^{\mu\nu}
\end{equation}
which is the standard chiral anomaly.


\subsection{Theoretical Summary}

We have seen above that a consistent quantum field theory requires
modification of the naive short distance behavior and leads to the
breaking of axial symmetry---
\begin{equation}
\partial^\mu J^3_{5\mu}=F_\pi m_{\pi^0}^2\phi_{\pi}^3+{e^2\over 16\pi^2}F_{\mu\nu}\tilde{F}^{\mu\nu}
\end{equation}
This anomalous symmetry breaking leads to a decay rate
\begin{equation}
\Gamma^{anom}_{\pi\rightarrow\gamma\gamma}=7.76\,\,{\rm eV}
\end{equation}
When real world corrections such as chiral symmetry breaking and
mixing are included this prediction is raised by about 4.5\% to
\begin{equation}
\Gamma^{theo}_{\pi\rightarrow\gamma\gamma}=8.10\,\,{\rm eV},
\end{equation}
with remarkably little theoretical uncertainty.  An ${\cal
O}(1\%)$ experimental verification of this prediction would then constitute a
validation of QCD.

Although rigorous quantum field theoretical arguments lead unambiguously to this
violation of axial symmetry, it is also useful to understand the
"physics" of this phenomenon and we presented arguments which show
that origin of the anomaly is the modification of the vacuum state of the field theory
in the presence of an electromagnetic field.  Having then understood the connection of
the decay rate of the $\pi^0$ with QCD, we move now to examine the experiments.

%\end{document


